InF-ATPG: Intelligent FFR-Driven ATPG with Advanced Circuit Representation Guided Reinforcement Learning

Automatic test pattern generation (ATPG) is a crucial process in integrated circuit (IC) design and testing, responsible for efficiently generating test patterns. As semiconductor technology progresses, traditional ATPG struggles with long execution times to achieve the expected fault coverage, which impacts the time-to-market of chips. Recent machine learning techniques, like reinforcement learning (RL) and graph neural networks (GNNs), show promise but face issues such as reward delay in RL models and inadequate circuit representation in GNN-based methods. In this paper, we propose InF-ATPG, an intelligent FFR-driven ATPG framework that overcomes these challenges by using advanced circuit representation to guide RL. By partitioning circuits into fanout-free regions (FFRs) and incorporating ATPG-specific features into a novel QGNN architecture, InF-ATPG enhances test pattern generation efficiency. Experimental results show InF-ATPG reduces backtracks by 55.06\% on average compared to traditional methods and 38.31\% compared to the machine learning approach, while also improving fault coverage.

==> DATE25-InF-ATPG-sub/doc/abstract.tex <==

\begin{abstract}
    % Automatic test pattern generation (ATPG) is essential for integrated circuit (IC) testing, tasked with producing test patterns to achieve high fault coverage. 
    % As semiconductor technology advances, traditional ATPG algorithms struggle with insufficient fault coverage and long execution times, necessitating optimization.
    Automatic test pattern generation (ATPG) is a crucial process in integrated circuit (IC) design and testing, responsible for efficiently generating test patterns.
    As semiconductor technology progresses, traditional ATPG struggles with long execution times to achieve the expected fault coverage, which impacts the time-to-market of chips.
    Recent machine learning techniques, like reinforcement learning (RL) and graph neural networks (GNNs), show promise but face issues such as reward delay in RL models and inadequate circuit representation in GNN-based methods. 
    In this paper, we propose InF-ATPG, an intelligent FFR-driven ATPG framework that overcomes these challenges by using advanced circuit representation to guide RL. By partitioning circuits into fanout-free regions (FFRs) and incorporating ATPG-specific features into a novel QGNN architecture, InF-ATPG enhances test pattern generation efficiency. 
    Experimental results show InF-ATPG reduces backtracks by 55.06\% on average compared to traditional methods and 38.31\% compared to the machine learning approach, while also improving fault coverage.
    %while improving fault coverage slightly. %by 0.12\%.
\end{abstract}
    % ====== old version
    \iffalse
    Automatic test pattern generation (ATPG) is essential for integrated circuit (IC) testing and design for test (DFT), tasked with generating test patterns to achieve high fault coverage.
    As semiconductor technology advances and chip complexity increases, traditional ATPG algorithms struggle with insufficient fault coverage and long execution times, elevating the need for optimization.
    Although recent applications of machine learning techniques, such as reinforcement learning (RL) and graph neural networks (GNNs), show promise in addressing these challenges,
    they remain in their infancy, suffering from issues like reward delay in RL models and inadequate circuit representation in GNN-based methods.
    In this paper, we propose InF-ATPG, an intelligent FFR-driven ATPG framework that uses an advanced circuit representation guiding the RL approach to overcome these limitations.
    By partitioning circuits into fanout free regions (FFRs) to reduce decision sequence length and incorporating ATPG-specific features such as circuit logic states and SCOAP controllability/observability into a novel QGNN architecture,
    InF-ATPG significantly improves test pattern generation efficiency. %and fault coverage. 
    Experimental results show that InF-ATPG reduces backtracks by 55.06\% on average compared to the traditional gate-level ATPG method, and by 38.31\% on average compared to the unimproved machine learning method,
    while improving 0.12\% on average fault coverage.
    \fi


%Experimental results show that InF-ATPG reduces backtracks by up to 80\% over traditional methods, while improving fault coverage .
%Experimental results across multiple benchmark circuits demonstrate that InF-ATPG reduces backtracks by up to 55\% compared to traditional gate-level ATPG methods and by 38\% compared to the unimproved machine learning approach, while improving fault coverage.

%Automatic Test Pattern Generation (ATPG) is vital for integrated circuit (IC) testing, but as chip complexity increases, traditional ATPG methods struggle with inefficiency and insufficient fault coverage. In this paper, we propose InF-ATPG, a novel framework that integrates Fanout Free Region (FFR) partitioning with a QGNN-based reinforcement learning (RL) approach to address these challenges. FFR partitioning reduces decision sequence length, mitigating the reward delay issue in RL, while QGNN enhances circuit state representation by incorporating key ATPG-specific features such as controllability and logic states. Experimental results across multiple benchmark circuits demonstrate that InF-ATPG reduces backtracks by up to 55\% compared to traditional gate-level ATPG methods and by 38\% compared to existing machine learning approaches. InF-ATPG also achieves an average fault coverage of 99.5\% and reduces decision sequence length by a factor of 6.8, showcasing its effectiveness in improving test generation efficiency and scalability.

% \begin{IEEEkeywords}
% ATPG, GNN, Reinforcement Learning, Design For Test, Machine Learning
% \end{IEEEkeywords}


==> DATE25-InF-ATPG-sub/doc/algo.tex <==
\section{InF-ATPG Framework}
\label{sec:algo}

%As the complexity of integrated circuit design increases, traditional machine learning-assisted ATPG algorithms face challenges such as long decision sequences, reward delay, and inadequate circuit state representation. These challenges hinder fault coverage and execution efficiency, making it difficult to meet the demands of modern chip designs. To address these issues, the InF-ATPG framework proposes an improved circuit partitioning strategy based on Fanout Free Regions (FFRs) and incorporates a Quality-Value Graph Neural Network (QGNN) agent with reinforcement learning (RL) to significantly improve test pattern generation efficiency and fault coverage.

To address the aforementioned challenges introduced by existing solutions, we propose the InF-ATPG framework, which employs a novel RL-based approach utilizing block-level circuit search spaces and ATPG-specific circuit representations. 
% By integrating an FFR-based partitioning strategy with a QGNN-driven agent, InF-ATPG significantly improves test generation efficiency and fault coverage.
\Cref{fig:inf-atpg} illustrates an overview of the InF-ATPG framework. Its key innovations are as follows:
% To address the challenges above, the InF-ATPG framework introduces a novel RL-based approach driven by block-level circuit search spaces and ATPG-specific circuit representations. By combining an FFR-based partitioning strategy with a QGNN-driven agent, it significantly enhances test generation efficiency and fault coverage.



%As IC design complexity grows, machine learning ATPG methods face challenges such as long decision sequences, reward delay, and inadequate state representation, limiting fault coverage and efficiency. To address these issues, the InF-ATPG framework introduces an FFR-based partitioning strategy combined with a Quality-Value Graph Neural Network (QGNN) driven agent and reinforcement learning, significantly improving test generation efficiency and fault coverage.

\begin{itemize}
    \item \textbf{Circuit partitioning and FFR backtrace (see \Cref{fig:inf-atpg}(a)):} %The circuit is divided into multiple FFRs, where each FFR serves as the smallest decision-making unit. This partitioning strategy simplifies and shortens the decision sequence, reducing redundant decisions and effectively alleviating reward delay in large-scale circuits. 
    % The circuit is partitioned into FFRs, each serving as the smallest decision-making unit. This reduces decision sequence length and mitigates reward delay by eliminating redundant decisions. Further elaboration on this aspect is provided in Section~\ref{3.1}.
    We first partition the circuit into Fanout-Free Regions (FFRs), which serve as the smallest decision-making units. This partitioning reduces the decision sequence length and mitigates reward delay by eliminating redundant decisions. Further details are provided in Section~\ref{3.1}.

    
    \item \textbf{QGNN-based state representation (see \Cref{fig:inf-atpg}(b)):}
    % A customized QGNN architecture is introduced, where the GNN serves as the RL agent. It represents the state of FFR-based sub-circuits, enhancing the generalization ability of the RL process. Further elaboration on this aspect is provided in Section~\ref{3.2}. 
    % We present a customized QGNN architecture, designed to function as the RL agent by representing the states of FFR-based sub-circuits. QGNN improves the RL process’s generalization capability by effectively capturing circuit-level features. Further details are discussed in Section~\ref{3.2}.
    While reducing decision length improves efficiency, it is essential to represent circuit states accurately to ensure correct decisions. To this end, we introduce a customized Quality-Value Graph Neural Network (QGNN) architecture, which captures critical features of FFR-based sub-circuits. QGNN enhances the RL agent's generalization ability by learning complex relationships between circuit elements. Further details are discussed in Section~\ref{3.2}.
    
    \item \textbf{MDP process and DQN modeling (see \Cref{fig:inf-atpg}(c)):} 
    % Based on FFR partitioning and QGNN state representation, %the InF-ATPG framework models the ATPG problem as a Markov Decision Process (MDP). 
    % the ATPG problem is modeled as a Markov decision process (MDP). 
    % Key circuit state features are selected, and a DQN method is employed to evaluate the action values of selecting different fanin gates of each FFR. The agent is trained to optimize ATPG by selecting the optimal actions in each FFR, thereby improving test efficiency. Further elaboration on this aspect is provided in Section~\ref{3.3}.
    Building on the FFR partitioning and QGNN representation, we model the ATPG task as a Markov decision process (MDP). Key circuit state features are extracted, and a Deep Q-Network (DQN) is used to evaluate the action values of selecting different fanin gates within each FFR. Further elaboration on this aspect is provided in Section~\ref{3.3}.
\end{itemize}


\subsection{Circuit Partitioning and FFR-Level Backtrace}\label{3.1}

Traditional ATPG algorithms encounter challenges such as long decision sequences and reward delay, particularly in large-scale circuits. To address these issues, the InF-ATPG framework adopts a partitioning strategy based on FFRs. 


\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.92\linewidth]{DATE25-InF-ATPG-sub/pic/3_1_V2.pdf}
    \caption{Comparison of FFR-level and Gate-level backtrace. FFR-level backtrace shortens the decision sequence by directly targeting fanin gates, while Gate-level backtrace involves a longer sequence of intermediate gates.}
    \label{fig:ffr_backtrace}
\end{figure}

An FFR, a circuit sub-block with non-overlapping internal logic and a single output, encapsulates a self-contained unit of logic. This structure simplifies the decision-making process while providing a higher-level abstraction of the circuit by isolating the logic within the FFR.
% An FFR is a circuit sub-block with non-overlapping internal logic and a single output node. Cross-layer circuit partitioning can shorten the decision sequence, potentially revealing broader structural information beyond the gate level. This structure simplifies the decision-making process by isolating logic within the FFR, allowing for more efficient test pattern generation.
As shown in \Cref{fig:ffr_backtrace}, FFR-level backtrace significantly reduces the decision sequence length compared to gate-level backtrace. The gate-level backtrace from the output gate \textit{8} to the fanin gate \textit{1} requires traversing multiple gates (i.e., gate \textit{6}, or gates \textit{7} to \textit{4}), resulting in a longer decision sequence (length 2 or 3). In contrast, FFR-level backtrace directly targets the fanin gates of the FFR, reducing the sequence to a length of 1 by bypassing intermediate gates and directly focusing on the higher-level structure of the circuit.

%By partitioning the circuit into FFRs, InF-ATPG reduces decision-making complexity and addresses reward delay. 
By extracting each FFR in the circuit and its associated fanin gates to form a sub-circuit, InF-ATPG reduces the complexity of decision-making and solves the problem of reward delay.
Each FFR becomes the smallest decision unit, allowing the framework to generate test patterns more efficiently than traditional gate-level approaches.

\subsection{QGNN-based State Representation}\label{3.2}

In RL, accurately representing the logic state of circuits is a key challenge, especially when ATPG problems are modeled as partially observable Markov decision processes (POMDPs). The precision of state modeling directly impacts the generalization ability of the RL model. Traditional ATPG methods primarily focus on individual gate characteristics, which limits their ability to capture complex circuit relationships, thereby affecting overall performance. To address this, the InF-ATPG framework introduces a customized quality-value graph neural network (QGNN) architecture. 
QGNN captures ATPG-specific features and introduces a logic-value-aware multi-aggregator design based on GAT\cite{velickovic2017graph}, enabling a more precise representation of the action's Q-value.  
% QGNN is specifically designed to capture the local fanout and reconvergent structures within circuits, providing enhanced state representation and improving the model's understanding of circuit logic.

\minisection{Circuit-Logic-State Features}
QGNN utilizes a variety of key circuit features to construct a comprehensive state representation, as shown in \Cref{tab:qgnn-features}.
The logic value directly reflects circuit functionality, while the objective value guides decision-making by adjusting targets. SCOAP controllability and observability quantify the difficulty of controlling and observing a node.
These features capture both the static and dynamic characteristics of circuit states that are essential for ATPG, enabling QGNN to model essential circuit logic states more effectively than heuristic methods. QGNN generates a more robust state representation, significantly enhancing the RL agent’s ability to make optimal decisions during ATPG.
\begin{table}[tb!]
    \centering
    \caption{Key circuit features in QGNN state representation}
    \resizebox{.99\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
        \textbf{Feature} & \textbf{Description} \\ \hline \hline
        Logic Value      & The logic value of the node (i.e., 0, 1, X) \\ \hline
        Objective Value  & Expected logic value for objective gate (in PODEM) \\ \hline
        SCOAP Controllability & Measures if the node can be controlled by PIs \\ \hline
        SCOAP Observability   & Measures if the node can be observed at a PO \\ \hline
        Gate Type        & One-hot encoded type of the logic gate \\ \hline
        \#Fanout         & Number of fanout gates connected to the node \\ \hline
        Depth            & Depth of the node from the PIs \\ \hline
    \end{tabular}
    }
    \label{tab:qgnn-features}
\end{table}
% The features capture both the static and dynamic circuit logic characteristics essential for ATPG.
% These features enable QGNN to model essential circuit logic states more effectively than heuristic methods, which often overlook such detailed properties. Considering factors such as logic value, controllability, and observability, QGNN generates a more robust state representation, significantly enhancing the RL agent’s ability to make optimal decisions during ATPG.

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.92\linewidth]{DATE25-InF-ATPG-sub/pic/QGNN_V2.pdf}
    \caption{QGNN aggregation process across different logic states in an FFR. Nodes with 0, 1, and X logic values use different aggregators to propagate information, enhancing the model's ability to capture complex circuit dependencies.}
    \label{fig:qgnn_model}
\end{figure}


\minisection{QGNN Model}
QGNN models each FFR and its fanin gates as a graph, where each logic gate is represented as a node, and edges represent the connections between gates. As illustrated in \Cref{fig:qgnn_model}, the model assigns an embedding vector (e.g., $h_1$, $h_2$, $h_3$) to each node, encoding its features. These embeddings are then updated through message aggregating and passing using a GAT, which aggregates information in the reverse direction of circuit computation, layer by layer.
The aggregation process is governed by the following equations:
\begin{equation}
\begin{split}
    \alpha_{ij} &= softmax_{j}((\vec{W}_q \vec{h}_i)^\top \cdot (\vec{W}_k \vec{h}_j)), \\
    \vec{m}_j &= \vec{W}_v \vec{h}_j  \label{eq:alpha_ij}, \\
    \vec{msg}_i &= aggr(\vec{h}_j \mid j \in P(i)) = \sum_{j \in P(i)} (\alpha_{ij} \cdot \vec{m}_j), %\label{eq:msg_i}
\end{split}
\end{equation}
where $P(i)$ represents the predecessors of node $i$, $\alpha_{ij}$ represents the attention weight between node $i$ and node $j$, and $\vec{W}_q$, $\vec{W}_k$, $\vec{W}_v$ are the weight matrices of the aggregator. The aggregated message $\vec{msg}_i$ is then passed to a gated recurrent unit (GRU) to update the node's embedding:
\begin{equation}
    \vec{h}_i \leftarrow{ \text{GRU}(\vec{h}_i, aggr(\vec{h}_j \mid j \in P(i)))}.
\end{equation}

This process allows QGNN to capture the complex dependencies between nodes in the circuit, ultimately producing final embeddings for the target FFR. These embeddings provide rich information for the RL agent to select optimal actions during ATPG.

\minisection{Innovative Aggregator Design}
One of the key innovations in QGNN is the use of multiple aggregators tailored to different logic states ($0$, $1$, $X$).
As shown in \Cref{fig:qgnn_model}, different aggregators ($\text{aggr}_0$, $\text{aggr}_1$, $\text{aggr}_X$) are applied depending on the logic value of the node.
This design ensures that the information flow is adapted to the specific logic state of each node, allowing for more precise information propagation.
The aggregation functions for different logic states are defined as follows:
\begin{equation}
\begin{split}
\text{0-aggr} &\rightarrow \text{GRU}_{logic0}(\vec{h}_i, aggr_{logic0}(\vec{h}_j \mid j \in P(i))), \\
\text{1-aggr} &\rightarrow \text{GRU}_{logic1}(\vec{h}_i, aggr_{logic1}(\vec{h}_j \mid j \in P(i))), \\
\text{X-aggr} &\rightarrow \text{GRU}_{logicX}(\vec{h}_i, aggr_{logicX}(\vec{h}_j \mid j \in P(i))). \\
\end{split}
\end{equation}

This design is critical because nodes with different logic values (i.e., 0, 1, X) often exhibit different signal propagation behaviors. By decoupling the aggregation processes for different logic states, QGNN ensures that the information relevant to each state is processed independently, improving the expressiveness of the model.

\subsection{MDP and DQN Modeling}\label{3.3}
Building on FFR partitioning and QGNN-based state representation, the InF-ATPG framework models the ATPG problem as an MDP and incorporates a tailored DQN framework to train the QGNN-driven RL agent for optimal action selection.

\minisection{MDP Modeling}
To enable the RL agent to navigate the complexities of circuit testing effectively, the key elements of the MDP include:
\begin{itemize}
    \item \textbf{State:} The state is defined by the logic state and circuit features of each FFR. The QGNN generates embedding vectors that represent the state of each FFR in the circuit.
    \item \textbf{Action:} Based on the QGNN state embeddings, the RL agent selects actions, which involve choosing a fanin gate in each FFR for the backtrace process. The action space is unified across FFRs regardless of the number of fanins.
    \item \textbf{Reward:} The reward function is designed to reduce backtracks and prioritize critical primary inputs (PIs), thereby accelerating test generation. 
    \circled{1}The reward function penalizes unnecessary decisions with a small negative reward (-0.1). 
    \circled{2}When reaching a PI, the reward function assigns rewards based on the frequency of this PI's visits and the number of backtracks encountered between assigning a value to this PI and the next backtrace step. By this, we impose immediate penalties on conflicting PIs and avoid redundant visits. 
    % assigns penalties or rewards based on the number of backtracks and visits to specific PIs. 
    \circled{3}If a test is successfully generated or the backtrack limit is exceeded, the episode ends with a corresponding reward, thereby aligning the training process with the objective of test generation:
\end{itemize}
\[
%\centering
\text{Reward} =
\begin{cases} 
-0.1, & \text{if not reach PI}; \\
10 - \lambda_1 \cdot e^{\lambda_2 \cdot N}, & \text{if reach PI}; \\
100, & \text{Test found/No test}; \\
-100, & \text{Over backtrack limit};
\end{cases}
\]
\[
 N = \#\text{backtracks}[\text{PI}] + \#\text{visits}[\text{PI}].
\]


\minisection{DQN Modeling}
The DQN process is illustrated in \Cref{fig:dqn_model}, and the key steps are as follows:
\begin{itemize}
    \item \textbf{Action Value Evaluation:} To enhance the effectiveness of circuit representation in RL-driven test generation, InF-ATPG employs the constructed QGNN alongside a multilayer perceptron (MLP) as the value network to guide the RL agent. This value network predicts the future value of all possible actions, with the action carrying the highest Q-value selected as the optimal choice.
    \item \textbf{Q-Value Update:} The QGNN and MLP are updated to minimize the loss between the predicted Q-values and the Q-targets. The Q-targets are computed using the target QGNN and target MLP, which is periodically updated.
    \item \textbf{Exploration-Exploitation Trade-off:} During training, exploration selects actions randomly to ensure the model explores diverse possibilities, while exploitation chooses actions based on the highest Q-value to optimize decision-making. The exploration rate starts high to encourage broad exploration and is gradually reduced as training progresses, shifting the model towards exploitation for more refined, optimal strategies.
    % \item \textbf{Exploration-Exploitation Trade-off:} During training, exploration encourages the model to try diverse actions, while exploitation leverages the knowledge gained to optimize decision-making. The balance between exploration and exploitation is dynamically adjusted through the exploration rate, promoting effective learning and convergence to an optimal strategy.
    % \item \textbf{Exploration-Exploitation Trade-off:} During training, the DQN balances exploration and exploitation by adjusting the exploration rate. As the model learns, more exploration is encouraged, followed by gradual convergence to an optimal strategy.  
\end{itemize}
% Based on the MDP formulation, InF-ATPG employs a Deep Q-Network (DQN) to train the RL agent for optimal action selection. The DQN process is illustrated in \Cref{fig:dqn_model}, and the key steps are as follows:
% Based on the MDP formulation, InF-ATPG employs a Deep Q-Network (DQN) method to train the QGNN and Multilayer Perceptron (MLP) for optimal action selection. The DQN process is illustrated in \Cref{fig:dqn_model}, and the key steps are as follows:

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.92\linewidth]{DATE25-InF-ATPG-sub/pic/3_3_V2.pdf}
    \caption{MDP and DQN process in InF-ATPG. The QGNN generates state embeddings, and the DQN evaluates action values, selects actions, and updates the model through reinforcement learning. Transitions are stored and sampled from a PER buffer to optimize learning efficiency.}
    \label{fig:dqn_model}
\end{figure}

% \begin{itemize}
%     \item \textbf{Action Value Evaluation:} 
%     % The DQN evaluates the action values (Q-values) based on the current QGNN-generated embeddings. The action with the highest Q-value is selected as the optimal action.
%     DQN evaluates the actions based on the current model-predicted Q-value. The action with the highest Q-value is selected as the optimal action.
%     \item \textbf{Q-Value Update:} 
%     % The Q-values are updated by minimizing the loss between the predicted Q-values and the target Q-values. The target Q-values are computed using the target QGNN, which is periodically updated from the main QGNN model.
%     The QGNN and MLP are updated to minimize the loss between the predicted Q-values and the Q-targets. The Q-targets are computed using the target QGNN and target MLP, which is periodically updated.
%     \item \textbf{Exploration-Exploitation Trade-off:} During training, the DQN balances exploration and exploitation by adjusting the exploration rate. As the model learns, more exploration is encouraged, followed by gradual convergence to an optimal strategy.
% \end{itemize}

The training process leverages a prioritized experience replay (PER) buffer, where transitions (state, action, reward, next state, done) are stored during interaction with the circuit environment. Over time, the DQN samples transition from the PER buffer to learn and update. The QGNN and MLP are continuously updated based on the loss, 
% new Q-values,
ensuring the RL agent improves its decision-making over time.




==> DATE25-InF-ATPG-sub/doc/conclu.tex <==
\section{Conclusion and Future Work}
\label{sec:conclu}

%We propose InF-ATPG, a novel framework that combines FFR partitioning with QGNN-agented Reinforcement Learning to address key challenges in ATPG, such as long decision sequences, reward delay and difficulty in circuit states representation. By leveraging FFR to simplify decision-making and QGNN to enhance circuit state representation, InF-ATPG effectively reduces the overall decision complexity and captures critical circuit features more accurately. %Experimental results demonstrate up to a 50\% reduction in backtracks compared to traditional and machine learning-based approaches, validating the framework’s efficiency and scalability in handling complex IC designs.
%Experimental results show a 55.06\% reduction in backtracks compared to traditional Gate-level methods and 38.31\% over unimproved machine learning-based approach. This validates InF-ATPG’s efficiency and scalability in handling complex IC designs.

\iffalse
In this paper, we introduce InF-ATPG, a novel RL-based ATPG approach that leverages block-level circuit search spaces and advanced ATPG-specific circuit representations. Modeling circuits at the FFR level effectively reduces decision sequence length, addressing reward delay issues commonly encountered in RL models. Additionally, integrating key circuit features into the QGNN framework improves the representation of circuit states and functionalities by decoupling the aggregation processes for different logic states. Experimental results demonstrate a 55.06\% reduction in backtracks compared to the traditional gate-level method and a 38.31\% reduction over the unimproved machine learning approach.
\fi

In this paper, we introduce InF-ATPG, a novel RL-based ATPG approach that leverages block-level circuit search spaces and advanced ATPG-specific circuit representations. By modeling circuits at the FFR level, we effectively reduce the decision sequence length, thereby addressing the reward delay issues commonly encountered in RL models. Furthermore, integrating key circuit features into the QGNN framework enhances the representation of circuit states and functionalities by decoupling the aggregation processes for different logic states. Experimental results demonstrate a 55.06\% reduction in backtracks compared to the traditional gate-level method and a 38.31\% reduction over the unimproved machine learning approach.

Future work could investigate the integration of more sophisticated reinforcement learning algorithms and additional circuit characteristics to further enhance the efficiency and accuracy of the ATPG process. Moreover, exploring efficient deployment strategies for these models within existing ATPG frameworks represents a compelling research direction that could significantly advance the practical applicability of AI-guided ATPG methods in industrial settings.


==> DATE25-InF-ATPG-sub/doc/intro.tex <==
\section{Introduction}

\begin{comment}
%{{{
Automatic test pattern generation (ATPG), as a search algorithm for logic circuits, plays a crucial role in design for test (DFT) by generating effective and compact test patterns \cite{b1,b2,b3}.
The primary objective of ATPG is to minimize the runtime while maintaining the quality and coverage of test patterns. Consequently, numerous heuristic approaches have been proposed to improve the performance of ATPG algorithms, including D-algorithm \cite{b4}, PODEM \cite{b5}, FAN \cite{b6} and other methods. These algorithms have proven effective when chip designs were relatively small and less complex. However, as the complexity of chip designs continues to increase, traditional heuristic methods for ATPG encounter significant challenges.



In modern digital design, 
This trend has led traditional ATPG methods to struggle in generating effective test patterns, as they must navigate a complex and high-dimensional search space that is often highly constrained and intricate. Fortunately, in recent years, researchers have discovered that machine learning (ML) algorithms, especially artificial neural networks (ANNs), hold significant potential in assisting ATPG algorithms to develop better decision-making strategies \cite{b6,b7,b8,b9,b10,b11,b12,b13,b14}. 
\begin{figure}[h]
    \centerline{\includegraphics[width=0.98\linewidth]{pic/Questions.pdf}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}
Specifically, recent work has focused on leveraging ANNs to guide the backtrace process of the PODEM algorithm. For example,  
Roy ${et\;al.}$ \cite{b12} employed ANNs to predict the probability that each line will not require backtracking. 
Pandey ${et\;al.}$ \cite{b13} utilized a supervised learning approach with various ML algorithms to make similar predictions. 
Li ${et\;al.}$ \cite{b14} modeled the ATPG process as a Markov process, utilizing reinforcement learning (RL) to explore the search space and applying graph neural networks (GNNs) to enhance the model's generalization capabilities. These methods have shown significant success in reducing the number of backtracks in PODEM. 

However, current ANN-based ATPG algorithms are highly dependent on training data, learning decision-making strategies exclusively from the training set. Even smartATPG \cite{b14}, which incorporates a RL framework, exhibits limited generalization capabilities. This limitation arises because the circuit state (i.e., the logic values of the nodes) changes dynamically as values are assigned to primary inputs (PIs) or pseudo-primary inputs (PPIs). Consequently, the decision-making environment during the backtrace process is continuously altered as ATPG algorithm advances, which poses challenges for the model to maintain consistent performance across varying circuit states. On the other hand, while ATPG can be effectively modeled as Markov process, representing RL states based solely on individual logic nodes result in a highly complex hidden Markov process, significantly complicating its resolution.

To fully harness the potential of RL, reduce the complexity of hidden Markov process, we have extended the PODEM algorithm. First, we enhance the PODEM algorithm by making decisions at the Fanout Free region (FFR) level instead of the individual logic gate level. This improvement is grounded in the understanding that within FFRs, the path from the root node to the fanin is unique, and critical backtrace decisions are made at the boundaries of FFRs rather than internally. 
Second, we meticulously designed a directed acyclic graph-based graph neural network (DAG-GNN) to extract features from FFRs and incorporate logic values into the node's feature representation. Under the DAG-GNN framework, the state representation for RL is significantly enhanced.
Finally, a RL algorithm is employed, with an effective reward function designed by incorporating immediate penalties for backtracks, aligning the reinforcement learning optimization with the path-search problem.

To end this, we propose a reinforcement learning-based ATPG framwork, FFR-Jump ATPG, which utilizes a customized graph neural network to enhance RL state representation. Our major contributions are listed as follows.


\begin{itemize}
\item We have introduced an innovative improvement to the PODEM algorithm, enabling it to make decisions at the granularity of FFRs. This approach is motivated by the observation that conducting backtrace at the FFR level enhances the algorithm's ability to capture the characteristics of local fanout reconvergence.
\item We propose a customized DAG-GNN for the feature representation of sub-circuits. By leveraging this specialized GNN, we effectively embed node features and states into a latent space, allowing the model to capture invariant local characteristics despite the dynamic changes in circuit states.
\item We model the ATPG algorithm as a Markov process and employ a RL algorithm to explore the circuit search space. By designing a customized GNN to encode circuit states and incorporating an effective reward function with immediate penalties for backtracks, our RL approach can effectively learn the optimal path during the backtrace process.
\item Experimental results demonstrate that the FFR-Jump algorithm not only outperforms current ANN-based and heuristic algorithms on most benchmark circuits, but also shows significant superiority in online learning efficiency.
\end{itemize}

We organize the remainder of this paper as follows. Section II provides an overview of the relevant background. Section III details our proposed FFR-Jump ATPG framework, including the enhancements to the PODEM algorithm, the RL strategy implemented, and the GNN architecture employed. Section IV outlines the experimental setup and presents the results obtained from testing on various benchmark circuits. Finally, Section V concludes the paper.
%}}}
\end{comment}


%Automatic Test Pattern Generation (ATPG) plays a critical role in Integrated Circuit (IC) testing and Design-for-Testability (DFT). Its primary task is to generate efficient test pattern sets for specific fault models to achieve high fault coverage. However, as semiconductor technology advances into deep submicron processes, the complexity of chip design has significantly increased. Traditional heuristic algorithms face bottlenecks in fault coverage and execution time, leading to increasing demands for higher testing quality and cost. It has been reported that generating production test patterns with sufficient fault coverage can occupy more than 20\% of development time, and it may take over a month to complete. Therefore, optimizing ATPG algorithms has become an urgent challenge.

Automatic test pattern generation (ATPG) is crucial for integrated circuit (IC) testing and design for test (DFT), tasked with generating efficient test patterns to achieve high fault coverage~\cite{jang1995design,barnhart2001opmisr}. 
As semiconductor technology advances into deep submicron processes, the complexity of chip design has increased significantly~\cite{lavagno2017electronic,kamal2022silicon},
making the generation of test patterns that meet fault coverage requirements increasingly time-consuming~\cite{zhen2023conflict}.
It is indicated that generating test patterns with sufficient fault coverage can take over 20\% of development time, often exceeding a month~\cite{wang2006vlsi}.
Therefore, optimizing ATPG algorithms has become a pressing challenge~\cite{kunz2002sat,bushnell2004essentials}.


%In recent years, with the continuous progress in circuit representation methods and decision-making problem research, machine learning techniques have gradually emerged in ATPG. Although these techniques offer new approaches to certain ATPG challenges, their application is still immature and presents unresolved issues. For instance, SmartATPG attempted to use reinforcement learning (RL) to address decision-making problems in ATPG, but as shown in \Cref{fig:problem_figures}(a), the increasing circuit size leads to longer decision action sequences, causing the problem of reward delay. Additionally, the representation and extraction of circuit states are insufficient, as RL models fail to adequately capture the necessary circuit features, as depicted in Fig.~\ref{fig:problem_figures}(b). This leads to difficulties in training and convergence, with unsatisfactory results. Simultaneously, works like DeepGate2 and FGNN2 attempted to use Graph Neural Networks (GNNs) for representation learning of circuit functionality and states. However, these methods fail to fully consider the specific circuit characteristics in ATPG and DFT, and they do not incorporate key features from traditional ATPG into the representation framework, making it difficult to apply these methods directly to practical ATPG problems.

\begin{comment}
ATPG is a highly complex problem of finding signal assignments in the circuit space that satisfy complex constraints~\cite{chen2013two}.
While traditional methods rely on heuristics, recent learning-based models have improved search capabilities using accumulated data. 
Traditional approaches typically rely on heuristic algorithms, but recent efforts have introduced learning-based decision models to enhance searching efficiency through accumulated data, rather than human-driven optimizations. 
However, challenges remain in decision-making and representation. 
The first issue is delayed rewards: Smart-ATPG \cite{li2024smartatpg}, which uses reinforcement learning (RL) for gate-by-gate decisions, suffers from long decision chains as circuit depth increases, leading to delayed rewards and slow convergence. 
The second issue is the difficulty in representing decision values, where existing graph neural network (GNN) approaches such as [] [] [], fail to capture ATPG-specific features, such as logic states and objective values, limiting their effectiveness. 
\end{comment}

ATPG is a highly complex problem of finding signal assignments in the circuit space to satisfy specific constraints \cite{chen2013two}.
While traditional methods rely on heuristic algorithms, 
% recent advancements have introduced learning-based models aimed at enhancing searching capabilities through accumulated data rather than relying on ad-hoc optimizations based on human experience. 
recent advancements introduced learning-based models aimed at enhancing searching capabilities through accumulated data rather than relying on human-driven optimization. 
However, these intelligent models still face problems in decision-making and representation for ATPG tasks.
One major problem is delayed rewards: SmartATPG \cite{li2024smartatpg} uses reinforcement learning (RL) to make decisions gate-by-gate, as illustrated in \Cref{fig:problem-a}.
% As circuit depth increases, the decision chain of this gate-by-gate approach becomes excessively long, leading to reward delay and slow convergence. 
As the bandwidth and depth of the circuit increase, the fault support regions expand considerably, resulting in excessively long decision chains for gate-by-gate approaches. This elongation leads to delayed rewards and slow convergence in the optimization process.
Another key problem is the inadequate representation of decision values, where existing approaches like FGNN2 \cite{wang2024fgnn2} and DeepGate2 \cite{shi2023deepgate2} leverage graph neural networks (GNNs) to model circuit functionality and structure but fail to capture ATPG-specific features like logic states and SCOAP controllability/observability~\cite{goldstein1979controllability}. These logic states play a crucial role in ATPG algorithm decision-making, as illustrated in \Cref{fig:problem-b}. 
Thus, the main challenge for intelligent ATPG is how to efficiently represent circuits, including appropriate partitioning and state representation, to optimize RL decision-making and ensure critical ATPG-specific information is captured.
% Thus, the central challenge for intelligent ATPG models lies in efficiently representing circuits through appropriate partitioning and state modeling, ensuring that critical ATPG-specific information is fully captured to optimize RL-based decision-making.


\begin{comment}
ATPG is the problem of searching for a set of signal assignments in the circuit signal space that satisfy complex constraints, and it is NP-complete. Current traditional approaches primarily rely on heuristic algorithms to solve this search problem. Recently, some researchers have proposed learning-based decision models aimed at enhancing searching capabilities through accumulated data, rather than relying on ad-hoc optimizations based on human experience. However, for ATPG tasks, these intelligent models still face problems related to decision-making and representation.
The first problem is the delayed rewards in intelligent decision-making schemes. 
A recent intelligent framework, Smart-ATPG~\cite{li2024smartatpg}, uses reinforcement learning (RL) to make decisions gate-by-gate, as illustrated in \Cref{fig:problem-a}.
However, as circuit depth increases, the decision chain of this gate-by-gate approach becomes excessively long, leading to delayed rewards and making it difficult for the RL model to converge.
The second problem is the difficulty in representing decision values, i.e., effectively capturing the critical information of the circuit space. Recently, graph neural networks (GNNs) have been introduced to learn representations of circuit functionality, structure and state. However, as shown in \Cref{fig:problem-b}, existing approaches primarily focus on general tasks rather than ATPG,
thereby overlooking ATPG-specific characteristics, such as logic and objective values. 
As a result, the effectiveness of these methods in driving ATPG tasks has been significantly reduced.
Subsequently, from an EDA perspective, the main challenge for intelligent decision-making models for ATPG is efficiently representing circuits, including appropriate circuit slicing and state representation, to optimize RL decision steps and ensure that decision values fully capture ATPG-specific circuit information.
\end{comment}

\begin{comment}
    

ATPG要求在电路信号空间中搜索一组满足复杂约束的信号赋值，这是一个NPC的问题。当前的工业开发中主要依赖启发式算法求解这一搜索问题。近年来，一些研究者提出基于学习的决策模型，试图基于数据来增强模型决策能力，而不再赖人类经验对启发式算法进行ad-hoc优化。但对于电路ATPG任务，这些智能化模型仍然面临来自决策和相应的表示的挑战。
首先是智能化决策方案的奖励稀疏问题。最近的一个智能化算法使用RL gate-by-gate地进行决策，其过程如图1a所示。但是随着电路深度增大，smart-ATPG的决策链条会变得过长，使得奖励稀疏，导致RL模型难以收敛。
其次是对决策价值等的表示困难问题，让决策价值充分体现电路空间的多元信息。最近的研究如xx引入GNN对电路的功能、结构和状态进行表示学习。However, as shown in \Cref{fig:problem_figures}(b), existing works mainly target general tasks rather than ATPG, therefore overlooking certain circuit characteristics critical for ATPG, such as logic and objective value. As a result, the effectiveness of these tools in driving ATPG tasks has been significantly diminished.
因此，从EDA角度分析，智能化ATPG的主要挑战，是对电路的高效表示学习，即合理的电路切片以及对电路状态的表征，从而优化RL的决策步长，并使得决策价值充分体现ATPG-critical的电路信息。

\end{comment}

% Recently, machine learning techniques have shown promise in addressing certain ATPG challenges~\cite{huang2021machine}. Although they sometimes demonstrate clear advantages, they still face challenges in decision-making and corresponding representation for circuit ATPG.
% For instance, recently, SmartATPG uses reinforcement learning (RL) to solve ATPG's decision-making issues~\cite{li2024smartatpg}.
% However, as shown in \Cref{fig:problem_figures}(a), growing circuit size results in longer decision sequences, leading to reward delay and making RL model training and convergence difficult~\cite{graesser2022state}. 
% Simultaneously, some recent representative learning frameworks such as FGNN2~\cite{wang2024fgnn2} and DeepGate2~\cite{shi2023deepgate2} attempted to use Graph Neural Networks (GNNs) to learn %\jianandel{for representation learning of} 
% circuit functionality and states. However, as shown in \Cref{fig:problem_figures}(b), 
% existing works mainly target general tasks rather than ATPG, therefore overlooking certain circuit characteristics critical for ATPG, such as logic and objective value. As a result, the effectiveness of these tools in driving ATPG tasks has been significantly diminished.
% \jianan{In summary, the key challenges faced by existing learning-based ATPG methods remain the efficient representation and decision-making for large-scale circuits accompanied by diverse information}.


\begin{figure}[tb!]
    \centering
    \subfloat[]{ \includegraphics[width=0.50\linewidth]{DATE25-InF-ATPG-sub/pic/Questions-a_V2.pdf} \label{fig:problem-a}}
    \subfloat[]{ \includegraphics[width=0.50\linewidth]{DATE25-InF-ATPG-sub/pic/Questions-b_V2.pdf} \label{fig:problem-b}}
    \caption{Challenges in existing methods: (a) Long decision sequences lead to delayed rewards; (b) Inadequate circuit state representation for ATPG.}
    \label{fig:problem}
\end{figure}

\begin{comment}
因此，我们提出InF-ATPG，一个基于高效的电路表示的RL方案来对ATPG进行智能化决策。
为了优化RL决策链并捕获ATPG-specific feature，我们首先基于FFR对电路进行分块。基于FFR的分块是ATPG任务的最优子结构，无需块内搜索，导致block-level的方法，压缩了RL的决策链。同时地，FFR可以驱动推算每个分块的logic states and controllability，这是ATPG任务的重要信息。然后，为了充分表示学习这些逻辑数值，我们提出一个具有新颖的logic-value-aware multi-aggregator的Quality-Value Graph Neural Network (QGNN)。最后，我们将表征ATPG-specific信息的QGNN集成进block-by-blcok的RL模型，实现了超越传统方案的智能化ATPG模型。
\end{comment}

\begin{comment}
To this end, we propose InF-ATPG, an RL-based intelligent ATPG solution based on advanced circuit representations. 
% To optimize the RL decision chain and capture ATPG-specific features, we first partition the circuit based on Fanout-Free Regions (FFRs) with a single output and non-overlapping internal logic, allowing reducing decision sequences and capturing broader structural information beyond the gate level.
To optimize the RL decision-making process and capture ATPG-specific features, we first partition the circuit into Fanout-Free Regions (FFRs) with a single output and non-overlapping internal logic. This approach reduces the length of decision sequences and captures broader structural information beyond the gate level.
% FFR-based partitioning provides an optimal substructure for ATPG tasks, eliminating the need for intra-block search, thereby shortening the RL decision chain.
Simultaneously, FFRs derive the circuit's logic states and controllability, which are essential for ATPG tasks. 
Next, to learn representations of these logic values, we introduce a novel Quality-Value Graph Neural Network (QGNN) based on a logic-value-aware multi-aggregator. 
Finally, we use the QGNN, which captures ATPG-specific information, to optimize the representation of action values in RL, achieving an intelligent ATPG model that surpasses traditional approaches.
In summary, the paper makes several key contributions as follows: 
\end{comment}

\begin{comment}
To this end, we propose InF-ATPG, an RL-based approach that leverages block-level circuit search spaces and customized circuit representations specifically for ATPG. 
By partitioning circuits into fanout-free regions (FFRs) with a single output and non-overlapping logic~\cite{cong1994acyclic}, InF-ATPG reduces decision sequences and captures broader structural information beyond gate level. 
Building on the partitioned FFR-level circuit, InF-ATPG integrates key features such as logic states and SCOAP controllability/observability~\cite{goldstein1979controllability} to represent circuit states and functionality more accurately. This enables more effective GNN-based solutions for ATPG. 
% Rather than simply stacking GNNs, 
However, since simple GNNs cannot fully capture the importance of logic states, 
InF-ATPG introduces the quality-value graph neural network (QGNN), which employs a logic-value-aware multi-aggregator to capture the complex relationships between circuit structure and functionality. 
InF-ATPG integrates QGNN into the RL agent so that the enhanced representation allows the RL model to generate patterns more efficiently by offering deeper insight into circuit behavior.
In summary, the paper makes several key contributions as follows: 
\end{comment}


To this end, we propose InF-ATPG, an intelligent RL-based framework designed for efficient decision-making and representation in ATPG tasks. To enhance model performance, we extract broader circuit information by partitioning circuits into fanout-free regions (FFRs)~\cite{cong1994acyclic}, which reduces decision sequence length and captures higher-level structural insights. This abstraction integrates ATPG-specific features like logic states and SCOAP controllability/observability~\cite{goldstein1979controllability}, providing a more accurate representation of circuit states. Since simple GNNs struggle to fully capture the complexity of logic states, we introduce the Quality-Value Graph Neural Network (QGNN), which uses a logic-value-aware multi-aggregator to model complex relationships between circuit structure and functionality. Integrating QGNN into the RL agent enhances behavior-value estimation, enabling more efficient test pattern generation by offering deeper insight into circuit behavior. In summary, the paper makes three key contributions as follows:

\begin{comment}
    
To address these challenges, we propose a better circuit partitioning method by grouping gates into fanout free regions (FFRs)~\cite{cong1994acyclic}.
FFRs, characterized by a single output and non-overlapping internal logic, allow us to model circuits with shorter decision sequences, reducing redundant decisions and alleviating reward delay, thereby improving RL model generalization.
Beyond partitioning, we identified key circuit states and features (such as logic states and SCOAP~\cite{goldstein1979controllability}) that are crucial to ATPG~\cite{chang2002atpg}. 
% By incorporating these into a novel GNN architecture, named QGNN (Quality-Value Graph Neural Network) , we enable more accurate representation learning for FFR regions. QGNN serves as the RL agent, capturing complex relationships between circuit structure and functionality, leading to more efficient test pattern generation.
To capture the complex relationships between the features, we proposed the QGNN (Quality-Value Graph Neural Network) architecture, a GNN model with logic-value-aware multi-aggregators specifically designed for ATPG problems. QGNN, as the RL agent, can better capture the complex relationships between circuit structure and functionality in ATPG, thereby generating more efficient patterns.

\end{comment}

\begin{comment}
    

Based on these innovations, we propose a new ATPG framework, InF-ATPG, which offers the following significant contributions:
\begin{enumerate}
    \item \textbf{Circuit modeling based on FFR:} To address the reward delay issue caused by long action sequences in RL, we propose modeling the circuit using FFR as the smallest unit, significantly reducing decision sequence length.
    \item \textbf{Optimization of circuit feature representation:} We selected key circuit states and features (such as controllability and real-time logic states) during the ATPG process and integrated them into the GNN representation learning framework, enabling the model to better adapt to ATPG problem-specific characteristics.
    \item \textbf{Introduction and improvement of the QGNN architecture:} We improved the GNN by proposing the QGNN architecture, specifically designed to capture the complex relationships between circuit structure and features in ATPG problems. QGNN acts as the reinforcement learning agent, enhancing training and inference performance.
    \item \textbf{Experimental results:} Experimental results show that InF-ATPG reduces backtracks by up to 50\% compared to traditional methods, and by up to 30\% compared to existing machine learning-based methods, while improving fault coverage. 
\end{enumerate}

\end{comment}
% Based on the innovations, we propose a new framework, InF-ATPG, which offers following significant contributions:
\begin{itemize}
% [leftmargin=*]
	% \setlength{\itemsep}{0pt}
	% \setlength{\parsep}{0pt}
	% \setlength{\parskip}{0pt}

    % \item We identify FFR partitioning as the fundamental building block for an intelligent ATPG decision model. FFR-based partitioning shortens the decision chain and derives ATPG-specific logic states.
    % \item We propose an improved GNN framework that leverages a logic-value-aware multi-aggregator to learn ATPG-specific logic states, thereby optimizing the action-value estimation in the RL model.

    \item InF-ATPG innovatively explores block-level circuit spaces for RL-based ATPG. To address reward delay from long decision sequences, circuits are modeled with FFRs as the fundamental units, significantly shortening the sequence length. 
    \item To optimize the circuit representation and tailor the RL agent for ATPG-specific tasks, InF-ATPG integrates key circuit states and features into the QGNN framework. By capturing structural and functional features more efficiently at the FFR level, QGNN drives RL agents to achieve superior training and inference performance through a logic-value-aware multi-aggregator design.
    \item Experimental results show that InF-ATPG reduces backtracking by an average of 55.06\% compared to the traditional gate-level ATPG method, and by 38.31\% compared to the existing machine learning approach. Additionally, it reduces the decision sequence length by a factor of 7.0.
\end{itemize}

\begin{comment}
1. 我们提出用FFR分块为基础构建智能ATPG决策模型。基于FFR的分区既压缩了决策链，也提供了ATPG必要的逻辑状态。
2. 我们提出QGNN来充分学习ATPG-specific的逻辑状态，从而优化RL模型的行为估值。通过一个新颖的聚合器，Inf-ATPG高效捕捉了ATPG-specifc逻辑状态的变化。


\end{comment}

\begin{comment}
    

\begin{enumerate}
    \item \textbf{FFR-based circuit modeling:} To mitigate reward delay from long decision sequences, we model circuits using FFRs as the smallest unit, significantly reducing sequence length.
    \item \textbf{Optimized circuit representation:} Key circuit states and features, including logic states and controllability, are incorporated into the GNN learning framework, better aligning with ATPG-specific requirements.
    \item \textbf{QGNN architecture:} The QGNN is designed to capture complex relationships between circuit structure and features, acting as the RL agent to improve training and inference performance.
    %\item \textbf{Experimental results:} InF-ATPG reduces backtracks by up to 50\% compared to traditional methods and up to 30\% over existing machine learning methods, while improving fault coverage.
    \item \textbf{Experimental results:} %InF-ATPG reduces backtracks by up to 55.06\% compared to traditional gate-level ATPG methods and by 38.31\% over unimproved machine learning approaches. Additionally, it achieves an average fault coverage of 99.5\%, while significantly reducing decision sequence length by a factor of 6.8, significantly improving efficiency across benchmark circuits.
    InF-ATPG reduces backtracks by an average of 55.06\% compared to traditional gate-level ATPG methods, and by an average of 38.31\% compared to the unimproved machine learning method. In addition, it significantly reduces the decision sequence length by a factor of 7.0.
\end{enumerate}

\end{comment}

%Through this framework, we provide new perspectives for addressing the complex circuit design problems faced in ATPG and demonstrate the potential and application prospects of machine learning in ATPG.




==> DATE25-InF-ATPG-sub/doc/prelim.tex <==
\section{Background and Related Work}
\label{sec:prelim}

% \begin{figure*}[tb!]
%     \centering
%     \includegraphics[width=0.92\linewidth]{DATE25-InF-ATPG-sub/pic/deepcell_overview.pdf}
%     \caption{
%         Overview of the InF-ATPG framework.
%         (a) Circuit partitioning into FFRs simplifies decision-making;
%         (b) QGNN-based state representation improves the RL agent’s ability to generalize;
%         (c) MDP and DQN modeling optimize test generation efficiency.
%     }
%     \label{fig:inf-atpg}
% \end{figure*}

% \begin{figure*}[tb!]
%     \centering
%     \includegraphics[width=0.92\linewidth]{DATE25-InF-ATPG-sub/pic/deepcell_arc.pdf}
%     \caption{
%         Overview of the InF-ATPG framework.
%         (a) Circuit partitioning into FFRs simplifies decision-making;
%         (b) QGNN-based state representation improves the RL agent’s ability to generalize;
%         (c) MDP and DQN modeling optimize test generation efficiency.
%     }
%     \label{fig:inf-atpg}
% \end{figure*}

\begin{figure*}[tb!]
    \centering
    \includegraphics[width=1.0\linewidth]{DATE25-InF-ATPG-sub/pic/InF-Jump ATPG_V2.pdf}
    \caption{
        Overview of the InF-ATPG framework.
        (a) Circuit partitioning into FFRs simplifies decision-making;
        (b) QGNN-based state representation improves the RL agent’s ability to generalize;
        (c) MDP and DQN modeling optimize test generation efficiency.
    }
    \label{fig:inf-atpg}
\end{figure*}

As the complexity of IC design increases, traditional ATPG methods face numerous challenges in handling complex circuits.
Researchers have proposed various solutions to address these challenges. This section briefly reviews traditional ATPG methods, previous AI-guided methods, and their applications in ATPG.

\subsection{Preliminary ATPG Strategies and Fanout-Free Region}

\minisection{ATPG}
Traditional ATPG algorithms use heuristic searches to generate test patterns for fault coverage.
% Roth's D-algorithm \cite{b4} pioneered ATPG, marking the beginning of the field. 
Roth proposed D-algorithm\cite{b4} for conducting searches on circuits.
Goel introduced the PODEM \cite{b5} algorithm with distance-from-primary-inputs heuristic, which significantly reduced the decision space. At the same time, Fujiwara and Shimono proposed the FAN \cite{b6} algorithm, which avoids conflicts through unique sensitization and multiple backtracing. Larrabee further improved test generation for complex circuits by introducing SAT-based solving techniques \cite{larrabee1992test, huang2022neural, drechsler2008acceleration}. 
Building on this, researchers subsequently introduced heuristic optimization methods such as Simulated Annealing \cite{bandyopadhyay1998simulated, corno1997saara}, but these traditional method still struggle with growing circuit complexity.

% \minisection{Circuit Partitioning}
%Fanout Free Regions (FFRs) have been widely applied as a circuit partitioning method. By dividing circuits into multiple Fanout Free sub-blocks, FFR simplifies the circuit model \cite{cong1994acyclic}.

\begin{comment}
\minisection{Block-Level Circuit}
Fanout-free regions (FFRs) are commonly used for efficient circuit partitioning. By decomposing a circuit into FFRs, each with signal paths confined to a single output, FFRs simplify circuit structure and facilitate optimization processes \cite{cong1994acyclic}. It reduces complexity by localizing signal dependencies, enabling efficient test generation.
\end{comment}

%\minisection{Block-Level Circuit Partitioning}
\minisection{Fanout-Free Region}
% To address the limitations of traditional approaches in handling complex circuits, partitioning methods like Fanout-Free Regions (FFRs) have been introduced.
Fanout-free regions (FFRs) decompose a circuit into sub-regions in which every gate, except for the FFR head, has a single fanout, 
% where each gate except fanout has only one output \cite{cong1994acyclic}, 
simplifying the internal dependencies of each block. This localized structure reduces decision complexity, allowing more efficient test generation by confining the search space within smaller, independent regions. It should be noted that the FAN \cite{b6} algorithm utilizes FFR. FAN avoids conflicts through reverse implications across multiple gates, making decisions at FFR roots through a voting mechanism. However, when the number of gates capable of reverse implication in the circuit is insufficient, performance degradation occurs.
% where all signal paths converge to a single output

% To overcome these challenges, partitioning techniques like Fanout-Free Regions (FFRs) have been adopted. FFRs divide a circuit into blocks where all signal paths converge to a single output \cite{cong1994acyclic}, simplifying circuit dependencies. This approach reduces the decision complexity by localizing signal interactions within each block, enabling more efficient test generation by narrowing the search space to smaller, independent regions.

\subsection{Machine Learning Techniques}

\minisection{Reinforcement Learning}
Reinforcement learning (RL) learns optimal policies through interaction with the environment, making it particularly suitable for tasks requiring sequential decision-making. Sutton and Barto laid the theoretical foundation for RL \cite{sutton1998reinforcement}, while Watkins and Dayan's Q-learning algorithm provided a classical approach to action selection in RL \cite{watkins1992q}. Recently, deep reinforcement learning (DRL) has combined deep neural networks with RL models, such as Mnih $et\ al.$'s deep Q-network (DQN) \cite{mnih2013playing}. Schaul $et\ al.$ introduced Prioritized Experience Replay (PER), %further 
improving DQN's training efficiency and convergence speed \cite{schaul2015prioritized}.

\minisection{Graph Neural Networks}
Graph neural networks (GNNs) aggregate node characteristics through message-passing mechanisms and have gained widespread application in graph processing tasks \cite{niepert2016learning}. GraphSAGE introduced inductive representation learning to enhance GNN performance on large-scale graphs \cite{hamilton2017inductive}. Veličković $et\ al.$ proposed the graph attention network (GAT), which employs attention mechanisms for more effective feature aggregation in graphs with complex interactions \cite{velickovic2017graph}.

\minisection{Representation Learning for Circuits}
Representation learning enables models to capture the complex relationships between logic elements in circuits. FGNN and FGNN2 employed pre-training on circuit logic to significantly improve representation accuracy \cite{wang2022functionality, wang2024fgnn2}. DeepGate series also incorporated functional characteristics to generalize to complex circuits \cite{li2022deepgate, shi2023deepgate2, shi2024deepgate3}. The circuit transformer maintained circuit equivalence to generate high-quality circuit representations \cite{licircuit}, highlighting the potential of circuit representation learning. However, these methods often overlook critical ATPG-specific circuit states and fail to incorporate key features from %traditional 
ATPG, limiting their direct application to ATPG problems.

\subsection{Machine Learning Applications in ATPG}

Recently, machine learning techniques, particularly the combination of deep learning and RL, have offered new solutions for ATPG. Roy $et\ al.$ proposed artificial neural networks to guide the decision-making process in ATPG\cite{b12}. SmartATPG used RL to automate test pattern generation \cite{li2024smartatpg}. HybMT proposed a machine learning algorithm based on a hybrid meta-predictor, which significantly improved test generation efficiency \cite{sarangihybmt}. The application of reinforcement learning in ATPG has further demonstrated machine learning's potential in improving test generation efficiency \cite{li2024smartatpg, li2023intelligent}.

However, as circuit size increases, these AI-guided methods still face challenges. Major issues include reward delay caused by long decision sequences and inadequate circuit state modeling, making RL model training and convergence more difficult and limiting their practical effectiveness in ATPG.




==> DATE25-InF-ATPG-sub/doc/result.tex <==
\section{Experimental Results}
\label{sec:result}

% To evaluate the effectiveness of the proposed InF-ATPG framework, we conducted comprehensive experiments on various benchmarks. 
% This section introduces the experimental setup, benchmark circuit selection, and detailed analysis of the results.
% To comprehensively evaluate the performance of the proposed InF-ATPG framework, we conducted systematic experiments on a variety of benchmark circuits. 
% This section details the experimental setup, benchmark circuit selection, and an in-depth analysis of the results, showcasing the advantages of InF-ATPG over traditional ATPG methods and unimproved machine learning-based techniques.

\subsection{Experimental Setup}

\begin{comment}
    %{{{
All experiments were conducted on a server with Intel Xeon E5-2650 v4 CPUs and 256 GB of RAM, running Ubuntu 20.04. The proposed InF-ATPG framework was implemented in Python, using TensorFlow for the QGNN-based reinforcement learning model, and standard ATPG tools were employed for baseline comparisons.
We selected a set of ISCAS and ITC benchmark circuits to evaluate the performance of InF-ATPG. These circuits vary in size and complexity, representing a diverse set of real-world scenarios to test the robustness of our framework. The chosen benchmarks include:
\begin{itemize}
    \item \textbf{ISCAS-85:} Includes circuits such as \textit{c432}, \textit{c499}, \textit{c880}, \textit{c1355}, \textit{c1908}, \textit{c2670}, \textit{c3540}, \textit{c5315}, and \textit{c7552}.
    \item \textbf{ISCAS-89:} Sequential circuits such as \textit{s420}, \textit{s1196}, \textit{s1423}, \textit{s5378}, and \textit{s9234}.
    \item \textbf{ITC-99:} Larger, industrial-scale circuits such as \textit{b14}, \textit{b17}, \textit{b20}, and \textit{b22}.
\end{itemize}

These circuits were chosen to test the scalability of our approach on both combinational and sequential circuits, as well as on small to large circuits.
    

All experiments were conducted on an Intel Xeon E5-2650 v4 processors and 256 GB of RAM, running Ubuntu 20.04. The experiments were designed to comprehensively evaluate the performance of InF-ATPG in comparison to traditional ATPG methods and unimproved machine learning-based approaches. In particular, the baseline methods include a standard gate-level ATPG heuristic based on PODEM and an FFR-level heuristic method also based on PODEM. Additionally, we compare against an FFR-level GNN-based approach without the QGNN enhancements introduced in our framework.

We selected benchmark circuits from the widely-used ISCAS-85, ISCAS-89, and ITC-99 suites, which provide a diverse range of circuit sizes and complexities. The smallest circuit in our experiments, \textit{c432}, contains 607 gates, while the largest circuit, \textit{s38417}, contains 19,768 gates. 
These benchmarks were chosen to evaluate the scalability and robustness of InF-ATPG in different circuits, covering a wide range of real-world situations in IC testing.
%These benchmarks were chosen to evaluate the scalability and robustness of InF-ATPG across both combinational and sequential circuits, covering a wide spectrum of real-world scenarios in integrated circuit testing.
The comparison methods were evaluated under the same experimental conditions to ensure fairness and consistency in performance measurements.
%}}}
\end{comment}

All experiments were performed on NVIDIA A100 GPU and Intel
Xeon Processor (Skylake, IBRS) @ 2.99GHz, running Ubuntu 20.04. The primary goal was to evaluate the performance of InF-ATPG in comparison to the traditional ATPG method and the unimproved GNN-based approach. 
% As baseline methods, we used a standard gate-level ATPG heuristic based on PODEM, an FFR-level heuristic also based on PODEM, and an FFR-level GNN approach without the QGNN enhancements introduced in our framework.
As baseline methods, we used a standard PODEM based on gate-level heuristic \cite{oATPG}, an improved PODEM based on FFR-level heuristic, and an FFR-level GNN approach without the QGNN enhancements introduced in our framework.

%Benchmark circuits were selected from the ISCAS-85 \cite{brglez1985neutral} and ISCAS-89\cite{brglez1989combinational} suites to cover a broad spectrum of circuit sizes and complexities. The smallest circuit, \textit{c432}, contains 607 gates, while the largest, \textit{s38417}, consists of 19,768 gates. %These benchmarks were chosen to assess the scalability and robustness of InF-ATPG across various real-world IC testing scenarios.
Benchmark circuits from the ISCAS-85 \cite{brglez1985neutral} and ISCAS-89 \cite{brglez1989combinational} suites were selected to cover a range of circuit sizes and complexities, from 607 gates (\textit{c432}) to 19,768 gates (\textit{s38417}). 
% These benchmarks evaluate InF-ATPG's scalability and robustness in real-world IC testing.
It is noteworthy that the benchmark circuits were synthesized from RTL code and fault injection was performed using the oATPG\cite{oATPG} fault injection algorithm (oATPG\cite{oATPG} inserts faults at the pins of each cell to comply with industrial-grade ATPG workflows). Consequently, these benchmarks differ from the standard ISCAS-85 and ISCAS-89 benchmarks in both circuits and faults.

For hyperparameters, the QGNN and MLP learning rate were set to 0.0001, with a discount factor $\gamma$ of 0.95. 
The capacity of the PER buffer was configured as 512$\times$1024. 
Through extensive experimental exploration and parameter sensitivity analysis, the reward function parameters $\lambda_1$ and $\lambda_2$ were ultimately determined to be 7.5 and 0.07.
To ensure fairness and consistency, all comparison methods were evaluated under identical experimental conditions. 

For training, we selected 100 challenging faults from each circuit and conducted 10 training epochs. The remaining faults were used as the test set, allowing us to rigorously evaluate the generalization and effectiveness of the InF-ATPG framework.
Due to differences in implementation languages—InF-ATPG being a Python/C++ hybrid and the open-source gate-level ATPG heuristic \cite{oATPG} implemented in C++—a direct comparison of CPU time would be unfair. 
% Therefore, we use the number of backtracks as an indirect metric to assess ATPG performance.
Therefore, when comparing InF-ATPG with other baselines, we exclusively use the number of backtracks as a proxy metric to evaluate ATPG performance. Conversely, we directly compare the CPU runtime improvements of heuristic-based FFR-level ATPG versus Gate-level ATPG. By examining both the reduction in the number of backtracks between InF-ATPG and other methods, and the CPU runtime reduction between FFR-level ATPG and Gate-level ATPG, we can demonstrate that InF-ATPG has potential to achieve superior results through AI methods based on FFR-level decision-making.

% Due to implementation language differences, with InF-ATPG using Python/C++ hybrid and the open-source gate-level ATPG heuristic\cite{oATPG} implemented in C++, direct CPU time comparison is unfair. Therefore, we use the number of backtracks as an indirect measure to reflect ATPG performance.

\subsection{Experimental Results and Analysis}

\begin{table*}[tb!]
\centering
\caption{%Performance Comparison of InF-ATPG with gate-level and FFR-level ATPG Approaches
Comprehensive Performance Comparison of InF-ATPG with Gate-level and FFR-level ATPG Approaches%: Backtracks, Backtrace Steps, and Fault Coverage
}
\label{tab:metrics}

\begin{subtable}{\textwidth}
\centering
  \resizebox{\textwidth}{!}{

\begin{tabular}{|lr|rr|rrrr|rrrr|rrrr|} % 12 columns
\hline
\multirow{2}{*}{Circuit} & \multirow{2}{*}{\#Gates} & \multicolumn{2}{c|}{{InF-ATPG}} & \multicolumn{4}{c|}{Gate-level~\cite{oATPG}} & \multicolumn{4}{c|}{FFR-level heuristic} & \multicolumn{4}{c|}{FFR-level GNN} \\
    & & {\#B-track} & {\#B-trace} 
    & \#B-track  & {Red1}(\%) & \#B-trace & {Red2}(\%) 
    & \#B-track  & {Red1}(\%) & \#B-trace & {Red2}(\%) 
    & \#B-track  & {Red1}(\%) & \#B-trace & {Red2}(\%) \\
\hline
\hline
% \midrule
c432 & 607 & \textbf{27017} & \textbf{39417} & 46422 & 41.80 & 50809 & 22.42 & 41458 & 34.83 & 46165 & 14.62 & 47447 & 43.06 & 51587 & 23.59 \\ 
c1908 & 1514 & \textbf{8414} & \textbf{10903} & 14617 & 42.44 & 22568 & 51.69 & 13058 & 35.56 & 21654 & 49.65 & 11372 & 26.01 & 19264 & 43.40 \\ 
c1355 & 1792 & \textbf{19519} & \textbf{35861} & 47679 & 59.06 & 63557 & 43.58 & 118609 & 83.54 & 133023 & 73.04 & 55033 & {64.53} & 68635 & 47.75 \\ 
c2670 & 2335 & 37277 & \textbf{41753} & 41222 & 9.57 & 60486 & 30.97 & 32979 & -13.03 & 46616 & 10.43 & \textbf{29301} & -27.22 & 44949 & 7.11 \\ 
c3540 & 3080 & \textbf{32374} & \textbf{40576} & 72348 & 55.25 & 83859 & 51.61 & 96705 & 66.52 & 107593 & 62.29 & 64676 & 49.94 & 73104 & 44.50 \\ 
s9234 & 3518 & \textbf{5406} & \textbf{19909} & 75294 & {92.82} & 90508 & 78.00 & 82638 & {93.46} & 100165 & 80.12 & 10623 & 49.11 & 24620 & 19.13 \\ 
s15850 & 7290 & \textbf{10295} & \textbf{10295} & 51085 & 79.85 & 69527 & {85.19} & 43268 & 76.21 & 61271 & {83.20} & 24861 & 58.59 & 42603 & {75.84} \\ 
s38417 & 19768 & \textbf{53341} & \textbf{79765} & 132197 & 59.65 & 185653 & 57.04 & 89792 & 40.59 & 136154 & 41.42 & 92706 & 42.46 & 146852 & 45.68 \\ 

\hline
\hline
{Average} & - & - & - & - & {55.06} & - & {52.56} & - & {52.21} & - & {51.85} & - & {38.31} & - & {38.38} \\


    %\midrule
    % \bottomrule
    \hline
    % \hline
  \end{tabular}
  }
  \end{subtable}

\vspace{8pt} % 控制两个表格之间的距离，可以根据需要调整




\begin{comment}
    

\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rr|rrrr|rrrr|rrrr|} % 12 columns
\hline
\multirow{2}{*}{Circuit} & \multirow{2}{*}{\#Faults} & \multicolumn{2}{c|}{{InF-ATPG}} & \multicolumn{4}{c|}{Gate-level~\cite{oATPG}} & \multicolumn{4}{c|}{FFR-level heuristic} & \multicolumn{4}{c|}{FFR-level GNN} \\
    & & {{\#Dec-Fault}} & {{FC(\%)}} 
    & \#Dec-Fault  & {Diff1}(\#) & FC (\%) & {Diff2}(\%). 
    & \#Dec-Fault  & {Diff1}(\#) & FC (\%) & {Diff2}(\%).
    & \#Dec-Fault  & {Diff1}(\#) & FC (\%) & {Diff2}(\%). \\
\hline
\hline
% \midrule

c432 & 1740 & \textbf{1720} & \textbf{98.85} & \textbf{1720} & 0 & \textbf{98.85} & 0.0 & \textbf{1720} & 0 & \textbf{98.85} & 0.0 & \textbf{1720} & 0 & \textbf{98.85} & 0.0 \\ 
c1908 & 4284 & \textbf{4275} & \textbf{99.79} & \textbf{4275} & 0 & \textbf{99.79} & 0.0 & 4273 & 2 & 99.74 & 0.05 & \textbf{4275} & 0 & \textbf{99.79} & 0.0 \\ 
c1355 & 4932 & \textbf{4929} & \textbf{99.94} & \textbf{4929} & 0 & \textbf{99.94} & 0.0 & 4891 & 38 & 99.17 & {0.77}& 4928 & 1 & 99.92 & 0.02 \\ 
c2670 & 6250 & \textbf{6143} & \textbf{98.29} & \textbf{6143} & 0 & \textbf{98.29} & 0.0 & \textbf{6143} & 0 & \textbf{98.29} & 0.0 & \textbf{6143} & 0 & \textbf{98.29} & 0.0 \\ 
c3540 & 8710 & \textbf{8647} & \textbf{99.28} & 8644 & 3 & 99.24 & 0.04 & 8638 & 9 & 99.17 & 0.10 & \textbf{8647} & 0 & \textbf{99.28} & 0.0 \\ 
s9234 & 6396 & \textbf{6392} & \textbf{99.94} & 6357 & 35 & 99.39 & {0.55} & 6354 & 38 & 99.34 & 0.59 & \textbf{6392} & 0 & \textbf{99.94} & 0.0 \\ 
s15850 & 13294 & \textbf{13290} & \textbf{99.97} & 13244 & {46} & 99.62 & 0.35 & 13248 & {42} & 99.65 & 0.32 & 13287 & 3 & 99.95 & 0.02 \\ 
s38417 & 36786 & \textbf{36770} & \textbf{99.96} & 36750 & 20 & 99.90 & 0.05 & 36761 & 9 & 99.93 & 0.02 & 36759 & {11} & 99.93 & {0.03} \\ 

\hline
\hline


{Average} & - & - & {99.50} & - & {+13} & 99.38 & {+0.12} & - & {+17} & 99.27 & {+0.23} & - & {+2} & 99.49 & {+0.01} \\
    %\midrule
    % \bottomrule
    \hline
  \end{tabular}
  }
\end{subtable}

\end{comment}



\begin{subtable}{\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|lr|rr|rrrr|rrrr|rrrr|} % 12 columns
\hline
\multirow{2}{*}{Circuit} & \multirow{2}{*}{\#Faults} & \multicolumn{2}{c|}{{InF-ATPG}} & \multicolumn{4}{c|}{Gate-level~\cite{oATPG}} & \multicolumn{4}{c|}{FFR-level heuristic} & \multicolumn{4}{c|}{FFR-level GNN} \\
    & & {\#UD-Fault} & {UFP(\%)} 
    & \#UD-Fault  & {Diff.}(\#) & UFP(\%) & {Imp.(\%)} 
    & \#UD-Fault  & {Diff.}(\#) & UFP(\%) & {Imp.(\%)} 
    & \#UD-Fault  & {Diff.}(\#) & UFP(\%) & {Imp.(\%)} \\
\hline
\hline
% \midrule

c432 & 1740 & \textbf{20} & \textbf{1.15} & \textbf{20} & 0 & \textbf{1.15} & 0.0 & \textbf{20} & 0 & \textbf{1.15} & 0.0 & \textbf{20} & 0 & \textbf{1.15} & 0.0 \\ 
c1908 & 4284 & \textbf{9} & \textbf{0.21} & \textbf{9} & 0 & \textbf{0.21} & 0.0 & 11 & 2 & 0.26 & 18.18 & \textbf{9} & 0 & \textbf{0.21} & 0.0 \\ 
c1355 & 4932 & \textbf{3} & \textbf{0.06} & \textbf{3} & 0 & \textbf{0.06} & 0.0 & 41 & 38 & 0.83 & 92.68 & 4 & 1 & 0.08 & 25.00 \\ 
c2670 & 6250 & \textbf{107} & \textbf{1.71} & \textbf{107} & 0 & \textbf{1.71} & 0.0 & \textbf{107} & 0 & \textbf{1.71} & 0.0 & \textbf{107} & 0 & \textbf{1.71} & 0.0 \\ 
c3540 & 8710 & \textbf{63} & \textbf{0.72} & 66 & 3 & 0.76 & 4.54 & 72 & 9 & 0.83 & 12.50 & \textbf{63} & 0 & \textbf{0.72} & 0.0 \\ 
s9234 & 6396 & \textbf{4} & \textbf{0.06} & 39 & 35 & 0.61 & 89.74 & 42 & 38 & 0.66 & 90.48 & \textbf{4} & 0 & \textbf{0.06} & 0.0 \\ 
s15850 & 13294 & \textbf{4} & \textbf{0.03} & 50 & 46 & 0.38 & 92.00 & 46 & 42 & 0.35 & 91.30 & 7 & 3 & 0.05 & 42.86 \\ 
s38417 & 36786 & \textbf{16} & \textbf{0.04} & 36 & 20 & 0.10 & 55.55 & 25 & 9 & 0.07 & 36.00 & 27 & 11 & 0.07 & 40.74 \\ 

\hline
\hline


{Average} & - & - & {\textbf{0.50}} & - & {+13} & 0.62 & {30.23} & - & {+17} & 0.73 & {42.64} & - & {+2} & 0.51 & {13.58} \\
    %\midrule
    % \bottomrule
    \hline
  \end{tabular}
  }
\end{subtable}

\vspace{0.36pt} % 表格和表注之间的距离

  \begin{tablenotes}[flushleft]
      \raggedright
 %  [leftmargin=*]
	% \setlength{\itemsep}{0pt}
	% \setlength{\parsep}{0pt}
	% \setlength{\parskip}{0pt}
  % \begin{itemize}
 % [leftmargin=*]
	% \setlength{\itemsep}{0pt}
	% \setlength{\parsep}{0pt}
	% \setlength{\parskip}{0pt}
   % \footnotesize
  \item \tabitem {Gate-level~\cite{oATPG}}: Gate-level PODEM algorithm using a distance-from-primary-inputs heuristic.
  \item \tabitem {FFR-level heuristic}: FFR-level PODEM algorithm using a distance-from-primary-inputs heuristic.
  \item \tabitem {FFR-level GNN}: FFR-level ATPG approach that utilizes unimproved GNN (without QGNN), enhancing with RL.
  \item \tabitem {\#B-track}: The total number of backtracks performed during ATPG.
  \item \tabitem {\#B-trace}: The total backtrace steps during ATPG refer to the process of tracing from the objective gate to PI.
  % \item \tabitem {\#Dec-Fault}: The number of detected faults in this method. \   \   \  
 % \   \  {FC(\%)}: Fault coverage in this method.  
  % \item \tabitem {Red1/Red2 (\%)}: Percentage reduction in the number of backtracks ({Red1}) and backtrace steps ({Red2}) compared to this method. Positive values indicate that the InF-ATPG approach achieved fewer backtracks and backtrace steps.
  % \item \tabitem {Diff1 (\#)/Diff2 (\%)}: The difference in the number of detected faults ({Diff1}) and fault coverage ({Diff2}) compared to this method. Positive values indicate improved fault detection and coverage.

  \item \tabitem {\#UD-Fault}: %Number of undetected faults in the method.
  Undetected faults number in the method. \   \   \   \ 
   {UFP(\%)}: %Percentage of undetected faults %relative 
   Undetected faults percentage
 to total %number of 
 faults in the method.  

\item \tabitem {Red1/Red2 (\%)}: Percentage reduction in the number of backtracks ({Red1}) and backtrace steps ({Red2}) compared to this method. Positive values indicate that the InF-ATPG approach achieved fewer backtracks and backtrace steps.

\item \tabitem {Diff. (\#)/Imp. (\%)}: The difference in the number of undetected faults ({Diff.}) and the improvement in UFP ({Imp.}) compared to this method. Positive values indicate a reduction in undetected faults and an improvement in UFP.
     
  % \end{itemize}
\end{tablenotes}
\end{table*}


\begin{table}[tb!]
    \centering
    \caption{CPU time comparison between FFR-level and gate-level ATPG}
    \label{tab:cpu_rumtimes}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{|c|c|c|c|}
            \hline
            {Circuit} & {FFR-level(ms)} & {Gate-level~\cite{oATPG}(ms)}& {CPU Time Red.(\%)} \\
            \hline \hline
            c432  & 221 & 117 & -88.89 \\ 
            c1908 & 112  & 91  & -23.07  \\ 
            c1355 & 705 & 243 & -190.12  \\ 
            c2670 & 221 & 209  & -5.74  \\ 
            c3540 & 1008 & 1028 & \textbf{1.95}  \\ 
            s9234 & 441  & 495 & \textbf{10.91} \\ 
            s15850 & 695  & 731  & \textbf{4.92}  \\ 
            s38417 & 1629 & 2667 & \textbf{39.20} \\ \hline 
            % \hline
            % Average & - & - & 7.0  \\
            % \hline
        \end{tabular}
        }
        \vspace{0.36pt} % 表格和表注之间的距离
        \begin{tablenotes}[flushleft]
            \raggedright
        \item \tabitem  {CPU Time Red.(\%)}: Reduction of CPU time by FFR-level ATPG, calculated as (Gate-level$-$FFR-level) / (Gate-level).

        
\end{tablenotes}
\end{table}


\begin{table}[tb!]
    \centering
    \caption{Decision sequence length comparison between InF-ATPG and gate-level ATPG}
    \label{tab:benchmark_circuits}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{|c|c|c|c|c|}
            \hline
            {Circuit} & {FFR Avg-Dep.} & {InF-ATPG} & {Gate-level~\cite{oATPG}}& {Ratio ($\times$)} \\
            \hline \hline
            c432    & 5.0 & \textbf{119234} & 1169414 & 9.8  \\ 
            c1908   & 5.9 & \textbf{89363}  & 549736  & 6.2  \\ 
            c1355   & 8.2 & \textbf{335034} & 1844036 & 5.5  \\ 
            c2670   & 4.8 & \textbf{173617} & 700113  & 4.0  \\ 
            c3540   & 6.2 & \textbf{289443} & 2371960 & 8.2  \\ 
            s9234   & 3.7 & \textbf{70286}  & 1104367 & 15.7 \\ 
            s15850  & 3.5 & \textbf{70669}  & 645829  & 9.1  \\ 
            s38417  & 3.9 & \textbf{266244} & 1521569 & 5.7  \\ \hline \hline
            Average & 5.2 & \textbf{176736} & 1238378 & 7.0  \\

            \hline
        \end{tabular}
        }
        \vspace{0.36pt} % 表格和表注之间的距离
        \begin{tablenotes}[flushleft]
            \raggedright
        \item \tabitem  {FFR Avg-Dep.}: Average depth of FFRs in the circuit.
        %\item \tabitem  {InF-ATPG Dec-Len.}: Decision sequence length for InF-ATPG, %representing the total number of decisions made during ATPG. representing number of decisions during ATPG.
        %\item \tabitem  {Gate-level Dec-Len.}: Decision sequence length for Gate-level heuristic PODEM\cite{oATPG}, showing the number of decisions in a conventional approach.
        \item \tabitem  {Ratio ($\times$)}: Reduction of decision sequence length by InF-ATPG, calculated as (Gate-level) / (InF-ATPG).
            % \end{itemize}
\end{tablenotes}

\end{table}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.92\linewidth]{DATE25-InF-ATPG-sub/pic/3_4_V2.pdf}
    \caption{Gate-level decision-making, constrained by single-gate information, results in suboptimal backtrace decisions. In this instance, with \textit{x7} assigned to 0, setting gate \textit{y} to logic 1 would require all inputs \textit{x1}-\textit{x6} to be 1. Conversely, FFR-level decision-making can identify that a single backtrace through gate \textit{x} efficiently achieves the objective gate's target.}
    \label{fig:pic_5}
\end{figure}

\begin{comment}
    %{{{ 
In this section, we present a detailed analysis of the experimental results, focusing on the key performance metrics: backtrack reduction, fault coverage, and decision sequence length. We also incorporate an ablation study to further investigate the contributions of individual components of the InF-ATPG framework. The results are compared across InF-ATPG, gate-level ATPG, and FFR-level ATPG approaches to highlight the effectiveness of the proposed method.

\subsubsection{Backtrack Reduction}

Table \ref{tab:metrics} demonstrates that InF-ATPG consistently reduces the number of backtracks across all benchmark circuits. On average, InF-ATPG achieves a 55.06\% backtrack reduction compared to gate-level ATPG and a 52.56\% reduction compared to FFR-level heuristic ATPG. These improvements are primarily attributed to the FFR partitioning strategy, which simplifies the decision-making process by breaking the circuit into smaller, independent sub-blocks. The partitioning reduces the length of decision sequences, leading to fewer backtracks.

The ablation study further confirms the importance of FFR partitioning. When FFR partitioning is removed, the backtrack count increases significantly, with the system reverting to gate-level complexity. This shows that the partitioning mechanism is critical in reducing computational overhead and improving test generation efficiency.

\subsubsection{Fault Coverage}

In terms of fault coverage, InF-ATPG consistently achieves high coverage across all circuits, as shown in Table \ref{tab:metrics}. On average, InF-ATPG achieves 99.5\% fault coverage, outperforming both gate-level and FFR-level heuristic approaches. The QGNN-based state representation plays a pivotal role in this improvement by capturing key circuit features such as controllability, observability, and logic states. This enables the reinforcement learning (RL) agent to better propagate faults and generate more effective test patterns.

The ablation study reveals that replacing the QGNN with a standard GNN diminishes fault coverage and increases backtracks. The QGNN's ability to model intricate circuit dependencies and logic relationships is crucial for achieving high fault detection rates. Without QGNN, the system struggles to represent the circuit state accurately, leading to degraded performance.

\subsubsection{Decision Sequence Length}

Table \ref{tab:benchmark_circuits} shows the decision sequence length comparison between InF-ATPG and gate-level ATPG. On average, InF-ATPG reduces decision sequence length by a factor of 6.8 compared to gate-level ATPG. This reduction is a direct result of the FFR partitioning strategy, which allows the decision-making process to be localized at the FFR level, significantly shortening the sequence of decisions required for test generation.

The ablation study highlights the critical role of the RL agent in decision optimization. When RL is replaced with heuristic methods, decision sequences become significantly longer, and the overall efficiency deteriorates. The RL agent, driven by the QGNN’s accurate state representation, enables the system to make informed decisions with fewer steps, demonstrating the importance of learning-based optimization in complex circuits.

\subsubsection{Summary of Results}

The experimental results clearly demonstrate the effectiveness of InF-ATPG in reducing backtracks, improving fault coverage, and shortening decision sequences. The ablation study emphasizes the importance of each component in the framework:
\begin{itemize}
    \item \textbf{FFR partitioning} is essential for simplifying decision-making and reducing backtracks.
    \item \textbf{QGNN-based state representation} significantly improves fault coverage and reduces unnecessary backtracks by capturing complex circuit logic.
    \item \textbf{Reinforcement learning} optimizes the decision-making process, reducing decision sequence length and enhancing overall efficiency.
\end{itemize}

Overall, the synergy between these components makes InF-ATPG a highly effective approach for addressing the challenges posed by modern, large-scale circuit designs.

This section presents an analysis of the experimental results, focusing on backtrack reduction, fault coverage, and decision sequence length. An ablation study is also included to highlight the contributions of key components in the InF-ATPG framework. We compare InF-ATPG with gate-level and FFR-level ATPG approaches to demonstrate its effectiveness.

\subsubsection{Backtrack Reduction}

As shown in Table \ref{tab:metrics}, InF-ATPG achieves an average backtrack reduction of 55.06\% compared to gate-level ATPG and 52.56\% compared to FFR-level ATPG. This improvement is largely due to the FFR partitioning strategy, which simplifies decision sequences by dividing the circuit into smaller, independent regions. 

The ablation study confirms the necessity of FFR partitioning. Without it, backtrack counts rise significantly, emphasizing its role in reducing computational complexity and improving test generation efficiency.

\subsubsection{Fault Coverage}

Table \ref{tab:metrics} also shows that InF-ATPG achieves an average fault coverage of 99.5\%, outperforming both gate-level and FFR-level approaches. The QGNN-based state representation is instrumental in this, as it accurately captures circuit features like controllability and logic states, allowing the RL agent to enhance fault detection.

Ablation results show that replacing QGNN with a standard GNN degrades fault coverage and increases backtracks, underscoring the importance of QGNN in modeling circuit dependencies and improving test pattern generation.

\subsubsection{Decision Sequence Length}

Table \ref{tab:benchmark_circuits} highlights that InF-ATPG reduces decision sequence length by a factor of 6.8 on average compared to gate-level ATPG. This reduction stems from FFR partitioning, which localizes decision-making at the FFR level, significantly shortening decision sequences.

The ablation study shows that removing the RL agent leads to longer decision sequences, demonstrating the RL agent’s role in optimizing decision-making and reducing computational overhead through more informed choices.


\subsubsection{Summary of Results}

The results confirm that InF-ATPG effectively reduces backtracks, improves fault coverage, and shortens decision sequences. The ablation study highlights the critical role of each component:
\begin{itemize}
    \item \textbf{FFR partitioning} reduces decision complexity and backtracks.
    \item \textbf{QGNN-based state representation} improves fault coverage by capturing complex circuit logic.
    \item \textbf{Reinforcement learning} optimizes decision-making, reducing decision sequences and improving efficiency.
\end{itemize}

Overall, the synergy of these components makes InF-ATPG highly effective for modern, large-scale circuit designs.
%}}}
\end{comment}

%The results demonstrate that InF-ATPG significantly reduces backtracks, enhances fault coverage, and shortens decision sequences. The ablation study underscores the importance of FFR partitioning in simplifying decision complexity, the QGNN-based state representation in capturing circuit logic for improved fault detection, and reinforcement learning in optimizing decision-making. The combined effect of these components makes InF-ATPG highly effective for large-scale, modern circuit designs.

% \subsection{Experimental Results and Analysis}



%In this section, we present a comprehensive analysis of the experimental results based on the two key performance metrics examined in our experiments: backtrack reduction and decision sequence length. The results are compared across InF-ATPG, gate-level ATPG, and FFR-level ATPG approaches, and are further divided into subsections for clarity.
This section presents a concise analysis of the experimental results focused on backtrack reduction and fault coverage improvement. 
Additionally, we conducted experiments to further validate our method's effectiveness by demonstrating the CPU runtime reduction of FFR-level compared to Gate-level approaches, as well as the decision sequence length reduction of InF-ATPG relative to Gate-level approaches.
% Additionally, we conducted experiments to further validate the effectiveness of our approach by demonstrating the reduction in decision sequence length. 
We compare InF-ATPG with gate-level and FFR-level ATPG approaches, and include an ablation study to highlight the contributions of key components.


% \minisection{Backtrack and Backtrace Reduction}

%Table \ref{tab:metrics} shows the performance comparison of InF-ATPG with gate-level and FFR-level ATPG approaches in terms of backtrack and backtrace steps. The proposed InF-ATPG framework achieves significant reductions in the number of backtracks and backtrace steps across all benchmark circuits. 

%On average, InF-ATPG reduces backtracks by 55.06\% compared to traditional gate-level ATPG and by 52.56\% when compared to the FFR-level heuristic method. The FFR-level GNN, without the QGNN enhancements, also performed worse than InF-ATPG, with InF-ATPG reducing backtracks by 38.31\% on average compared to this method. The backtrace steps show similar trends, with InF-ATPG achieving a 52.21\% reduction compared to gate-level ATPG, 51.85\% compared to FFR-level heuristics, and 38.38\% compared to FFR-level GNN.

%These reductions are primarily attributed to the FFR-based partitioning strategy, which simplifies decision-making by reducing the length of decision sequences. The QGNN’s enhanced state representation further assists the reinforcement learning (RL) agent in making more informed decisions, thereby avoiding unnecessary backtracks. The results clearly demonstrate the effectiveness of InF-ATPG in reducing computational complexity, which is critical for large-scale circuits.


%%%


%As shown in Table \ref{tab:metrics}, InF-ATPG significantly reduces backtracks and backtrace steps across all benchmark circuits. On average, InF-ATPG reduces backtracks by 55.06\% compared to gate-level ATPG and by 52.56\% compared to FFR-level heuristics. In comparison to FFR-level GNN without QGNN enhancements, InF-ATPG reduces backtracks by 38.31\% and backtrace steps by 38.38\%.

%These reductions stem from the FFR-based partitioning strategy, which simplifies decision-making by shortening decision sequences. The QGNN’s improved state representation further aids the RL agent in optimizing decisions, minimizing unnecessary backtracks. These results confirm InF-ATPG’s ability to reduce computational complexity, especially in large circuits.

\minisection{Backtrack and Backtrace Reduction}
%As shown in Table \ref{tab:metrics}, InF-ATPG achieves substantial reductions in backtracks and backtrace steps across benchmark circuits. 
As shown in the upper part of \Cref{tab:metrics}, InF-ATPG achieves a significant reduction in backtracks and backtrace steps in various circuits when controlling for different methods to achieve the same fault coverage.
% InF-ATPG achieves a significant reduction in backtracks and backtrace steps in various benchmark circuits when controlling for different methods to achieve the same fault coverage measurements backtrack and backtrace steps.
On average, InF-ATPG reduces backtracks by 55.06\% compared to gate-level heuristic ATPG\cite{oATPG} and by 52.21\% compared to FFR-level heuristic ATPG. Moreover, compared to FFR-level GNN without QGNN enhancements, InF-ATPG reduces backtracks by 38.31\% and backtrace steps by 38.38\%. The consistent improvements across different circuits underscore the robustness of the proposed method.

%The key factor driving these reductions is the FFR-based partitioning strategy, which effectively simplifies decision-making by breaking the circuit into smaller, independent sub-blocks. This reduces the length of decision sequences, thus minimizing the number of backtracks required to generate a complete set of test patterns. Moreover, the QGNN-enhanced state representation further aids the RL agent by providing more accurate information about circuit states, enabling it to make more informed decisions. Ultimately, these results demonstrate that InF-ATPG offers a significant reduction in computational complexity, which is especially crucial when dealing with large-scale circuits.

The FFR-based partitioning strategy simplifies decision-making by dividing circuits into smaller, independent subblocks, reducing decision sequence length and minimizing backtracks for ATPG. Additionally, the QGNN-enhanced state representation provides the RL agent with more accurate circuit information, enabling more informed decisions. This highlights InF-ATPG's ability to significantly reduce computational complexity, especially for large-scale circuits.



% \minisection{Fault Detection and Coverage}

%Table \ref{tab:metrics} also compares the fault detection capabilities and fault coverage (FC) of InF-ATPG with other methods. InF-ATPG consistently achieved high fault coverage across all circuits, with an average fault coverage of 99.5\%, outperforming both gate-level and FFR-level heuristic methods. The average fault coverage improvement compared to gate-level ATPG is +0.12\%, while the improvement over FFR-level heuristic methods is +0.2\%.

%The performance of InF-ATPG in fault detection can be attributed to the QGNN-based state representation, which captures key circuit features such as logic values, controllability, and observability. This allows the RL agent to identify and propagate faults more effectively, leading to higher fault coverage.

%%%

%InF-ATPG also excels in fault detection, achieving an average fault coverage of 99.5\% (Table \ref{tab:metrics}), outperforming both gate-level and FFR-level heuristics. The improvements in fault coverage—+0.12\% over gate-level ATPG and +0.2\% over FFR-level heuristics—are attributed to the QGNN-based state representation, which effectively captures circuit features like logic values, controllability, and observability, enabling more robust fault propagation and detection.
\minisection{Fault Detection and Coverage}
%InF-ATPG also demonstrates superior performance in fault detection, achieving an average fault coverage of 99.5\%, as shown in \Cref{tab:metrics}. 
% As shown in the lower part of \Cref{tab:metrics}, InF-ATPG also performs well in fault detection with an average fault coverage of 99.5\% when comparing fault coverage as in the same max-backtrack limit. 
% This represents a +0.12\% improvement over gate-level heuristic ATPG\cite{oATPG} and a +0.23\% improvement over FFR-level heuristic ATPG. These enhancements are largely due to the QGNN-based state representation, which captures crucial circuit features such as logic values, controllability, and observability. By leveraging this detailed state information, the RL agent is able to propagate faults more efficiently and generate more effective test patterns, leading to higher fault coverage.
As presented in the lower section of \Cref{tab:metrics}, under the same max-backtrack limit, 
InF-ATPG successfully detects hard-to-detect faults that other methods fail to detect. InF-ATPG achieves an average undetected fault percentage (UFP)
of 0.50\%. 
% InF-ATPG also performs well in fault detection, achieving an average undetected fault percentage (UFP) of 0.50\%.
% As presented in the lower section of \Cref{tab:metrics}, InF-ATPG also performs well in fault detection, achieving an average undetected fault percentage (UFP) of 0.50\% under the same max-backtrack limit. 
This represents a 30.32\% improvement compared to gate-level heuristic ATPG \cite{oATPG}, which has a UFP of 0.62\%, and a 42.64\% improvement over FFR-level heuristic ATPG, which has a UFP of 0.73\%.
% As shown in the lower part of \Cref{tab:metrics}, InF-ATPG also performs well in fault detection with an average undetected fault percentage (UFP) of 0.50\% when comparing fault coverage as in the same max-backtrack limit. 
% This marks a 30.32\% improvement over gate-level heuristic ATPG \cite{oATPG}, which has a UFP of 0.62\%, and a 42.64\% improvement over FFR-level heuristic ATPG, which has a UFP of 0.73\%. 

While the average improvement is notable, InF-ATPG shows particularly significant gains on larger circuits, such as \textit{s9234} and \textit{s15850}, where undetected faults were reduced by over 90\% compared to other methods.
These improvements are attributed to the QGNN-based state representation, which captures deeper circuit features, allowing RL agent to optimize test generation. 
% These improvements are driven by the QGNN-based state representation, which effectively captures deeper circuit features. This enables the RL agent to optimize fault propagation and test generation, leading to more efficient pattern generation and fewer undetected faults, especially in complex, large-scale circuits.
% As shown in \Cref{tab:metrics}, InF-ATPG achieves strong performance in fault detection, with an average undetected fault percentage (UFP) of 0.50\%. This marks a +0.12\% improvement over gate-level heuristic ATPG \cite{oATPG}, which has a UFP of 0.62\%, and a +0.23\% improvement over FFR-level heuristic ATPG, which has a UFP of 0.73\%. These improvements are primarily due to the use of QGNN-based state representation, which effectively captures key circuit features such as logic values, controllability, and observability. With this detailed state information, the RL agent is able to better identify and propagate faults, resulting in more efficient test pattern generation and reduced undetected faults. This leads to higher fault coverage across various circuit benchmarks.


%As shown in the lower part of \Cref{tab:metrics}, InF-ATPG also performs well in fault detection with an average fault coverage of 99.5\% when comparing fault coverage as in the same max-backtrack limit. This represents a +0.12\% improvement over gate-level ATPG (UFP of 0.62\%) and a +0.23\% increase compared to FFR-level heuristic ATPG (UFP of 0.73\%). While the average improvement is notable, InF-ATPG shows particularly significant gains on larger circuits, such as *s9234* and *s15850*, where undetected faults were reduced by over 90\% compared to other methods. These improvements are driven by the QGNN-based state representation, which effectively captures deeper circuit features—such as logic values, controllability, and observability. This enables the RL agent to optimize fault propagation and test generation, leading to more efficient pattern generation and fewer undetected faults, especially in complex, large-scale circuits.

\begin{comment}
\minisection{Fault Detection and Coverage}
As shown in \Cref{tab:metrics}, InF-ATPG achieves strong performance in fault detection, with an average undetected fault percentage (UFP) of 0.50\%. This marks a +0.12\% improvement over gate-level heuristic ATPG \cite{oATPG}, which has a UFP of 0.62\%, and a +0.23\% improvement over FFR-level heuristic ATPG, which has a UFP of 0.73\%. These improvements are primarily due to the use of QGNN-based state representation, which effectively captures key circuit features such as logic values, controllability, and observability. With this detailed state information, the RL agent is able to better identify and propagate faults, resulting in more efficient test pattern generation and reduced undetected faults. This leads to higher fault coverage across various circuit benchmarks.

\end{comment}


% \minisection{Decision Sequence Length Reduction}

%\Cref{tab:benchmark_circuits} presents the comparison of decision sequence lengths between InF-ATPG and gate-level ATPG. The decision sequence length is a critical factor in test generation, as shorter sequences lead to faster test generation and reduced computational overhead.

%On average, InF-ATPG reduces decision sequence length by a factor of 6.8 compared to gate-level ATPG. For example, in the case of circuit s9234, InF-ATPG reduced the decision sequence length by a factor of 15.7 compared to gate-level ATPG. This significant reduction can be attributed to the FFR partitioning strategy, which simplifies the circuit into smaller, manageable regions. By focusing the decision process at the FFR level, InF-ATPG is able to drastically reduce the number of decisions required for test generation.

%The improved efficiency in decision-making is further enhanced by the QGNN model, which provides a more accurate representation of the circuit state, allowing the RL agent to make more efficient decisions.



%%%

%\Cref{tab:benchmark_circuits} shows that InF-ATPG reduces decision sequence length by a factor of 6.8 on average compared to gate-level ATPG. In circuit s9234, for instance, decision sequence length is reduced by 15.7 times. These improvements are driven by FFR partitioning, which breaks the circuit into smaller regions, allowing the RL agent to focus decision-making at the FFR level and drastically reduce the number of decisions required for test generation.


\minisection{CPU Runtime}
As illustrated in \Cref{tab:cpu_rumtimes}, this experiment aims to demonstrate that although both approaches utilize distance-based heuristic methods, decision-making at the FFR-level yields superior results compared to Gate-level decision-making. Table 3 reveals that for larger-scale circuits, FFR-level decision-making contributes to a reduction in CPU runtime. For instance, in the \textit{s38417} circuit, FFR-level decision-making reduced runtime by 39.20\% compared to the Gate-level approach\cite{oATPG}. Conversely, \Cref{tab:cpu_rumtimes} indicates that for smaller-scale circuits, FFR-level decision-making incurs significant initialization overhead due to the computational requirements of FFR calculation, thus requiring longer CPU time compared to the Gate-level approach\cite{oATPG}.

FFR-level decision-making provides a broader perspective compared to Gate-level decision-making. As exemplified in \Cref{fig:pic_5}, to set the objective gate to logic 1, Gate-level decision-making tends to select gate \textit{y} with smaller logic depth. However, in this example, since \textit{x7} has already been assigned a value of 0, adjusting gate \textit{y} to 1 incurs a substantial cost (requiring \textit{x1}-\textit{x6} all to be set to 1). Consequently, selecting gate y for backtrace is not an optimal choice. In contrast, FFR-level decision-making has the opportunity to comprehensively consider the logical state and topological connectivity relationships at the subcircuit level, thereby recognizing that performing a backtrace through gate \textit{x} can achieve the objective gate's target more efficiently.



\minisection{Decision Sequence Length Reduction}
This experiment was designed to demonstrate the respective impacts of FFR and QGNN on reducing the decision sequence length.
\Cref{tab:benchmark_circuits} shows that InF-ATPG reduces decision sequence length by an average factor of 7.0 compared to gate-level ATPG\cite{oATPG}, with a notable reduction of 15.7 in the case of \textit{s9234}. 

This reduction stems from the FFR partitioning strategy, which simplifies the decision process by dividing the circuit into smaller, independent regions, each with an average FFR depth of 5.2. This coarse-grained approach reduces the complexity of decision sequences by focusing on broader, higher-level sub-circuits. 
% , rather than individual gates.
Also, %using FFRs obtains an average reduction of 7.0 which is larger than 5.2, enhancing decision quality by enabling the extraction of more comprehensive circuit information. 
InF-ATPG achieves an average reduction %in decision sequence length 
of 7.0, which surpasses the average FFR depth of 5.2. 
% This indicates an improvement in decision quality as it facilitates the extraction of more comprehensive circuit information.
Guided by QGNN’s enriched state representation, the RL agent leverages this broader context to make more informed decisions, reducing unnecessary steps, and further improving efficiency. This combination of coarse-grained partitioning and enhanced decision-making allows InF-ATPG to significantly shorten decision sequences, making it scalable for larger circuits.

\begin{comment}
\minisection{Decision Sequence Length Reduction}
\Cref{tab:benchmark_circuits} presents the decision sequence length comparison between InF-ATPG and gate-level ATPG\cite{oATPG}. On average, InF-ATPG reduces decision sequence length by a factor of 7.0 compared to gate-level ATPG\cite{oATPG}. For instance, in the case of \textit{s9234}, InF-ATPG reduces decision sequence length by a factor of 15.7. This significant reduction can be attributed to the FFR partitioning strategy with an average FFR depth of 5.2, which divides the circuit into smaller, manageable regions. By focusing the decision-making process at the FFR level, InF-ATPG drastically reduces the number of decisions needed for ATPG.%test generation.

The RL agent, guided by QGNN’s enhanced state representation, further improves decision efficiency. The RL agent learns to make optimal decisions with fewer steps, avoiding unnecessary actions. This results in shorter decision sequences and faster test generation, making InF-ATPG highly scalable for large circuits.
\end{comment}




%The results demonstrate that InF-ATPG significantly reduces backtracks, enhances fault coverage, and shortens decision sequences. The ablation study underscores the importance of FFR partitioning in simplifying decision complexity, the QGNN-based state representation in capturing circuit logic for improved fault detection, and reinforcement learning in optimizing decision-making. The combined effect of these components makes InF-ATPG highly effective for large-scale, modern circuit designs.

\iffalse
The results confirm that InF-ATPG significantly reduces backtracks, improves fault coverage, and shortens decision sequences. The ablation study highlights the importance of FFR partitioning in simplifying decision complexity, QGNN-based state representation in capturing circuit logic for better fault detection, and RL in optimizing decision-making. %The synergy of these components makes InF-ATPG highly effective for large-scale, modern circuit designs.
\fi
The results confirm that InF-ATPG substantially reduces backtracks, enhances fault coverage, and shortens decision sequences. The ablation study underscores the critical role of FFR partitioning in reducing decision complexity, the effectiveness of QGNN-based state representation in capturing circuit logic for improved fault detection, and the contribution of RL in optimizing decision-making.



==> DATE25-InF-ATPG-sub/setting-ieee.tex <==
% =============================================================
%         setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 10/2023
% =============================================================

\usepackage{blkarray}                                      % to support matrix
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}                                 % new algorithm package
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}        % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure}{\textbf{Output:}}        % Use Output in the format of Algorithm
\usepackage{graphicx}                                      % include pdf figures
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage[mathcal]{eucal}
\usepackage{mathrsfs}
\usepackage{booktabs}
\usepackage{enumerate}
\usepackage{multirow}
\iffalse
\usepackage[subrefformat=parens,farskip=0pt,justification=centering]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\fi
\usepackage{color}
\usepackage{cite}                                          % more citations in one bracket
\usepackage{comment}                                       % use comment
\usepackage{soul}                                          % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{etoolbox}                                      % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}                                           % nth command
\usepackage{bm}                                            % bm command
\usepackage{courier}
\usepackage{balance}
\usepackage{threeparttable}
\usepackage{xcolor,colortbl}
\usepackage{footnote}
\usepackage{listings}
\usepackage{setspace}                                      % setstretch{}
\usepackage[inline]{enumitem}

\usepackage{verbatim}
\usepackage[bookmarks=false]{hyperref}
\hypersetup{
    colorlinks = true,
    citecolor  = blue,
    linkcolor  = blue,
    urlcolor   = blue,
}
\usepackage{tikz}
\usetikzlibrary{patterns,snakes}
\usetikzlibrary{positioning,calc,fit,decorations.pathmorphing,shapes.geometric, shapes.gates.logic.US, calc}
\usetikzlibrary{arrows,arrows.meta,decorations.markings,shapes,shapes.arrows}
\usetikzlibrary{decorations,decorations.pathreplacing}
\usetikzlibrary{backgrounds}
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{scalefnt}
\pgfplotsset{compat=newest}
\usepackage{caption}
\usepackage{pifont}                                        % ding commend
\usepackage{cleveref}
\Crefformat{figure}{Fig.~#2#1#3}                           % "Fig.", instead of "Figure"
\Crefname{subfigure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\Crefformat{table}{TABLE~#2#1#3}                           % "TABLE", instead of "Table"
\captionsetup[table]{skip=2pt}
\captionsetup{labelsep=space}
\usepackage[figuresright]{rotating}
\iffalse                                                   % minted
\IfFileExists{minted_configuration.tex}{\input{minted_configuration.tex}}{\usepackage[outputdir=../]{minted}}
%\usepackage[outputdir=./]{minted}              % code highlight, w. "--shell-escape" in pdflatex
\setminted{linenos=true, escapeinside=@@, fontsize=\small, numbersep=8pt}
\usemintedstyle{lovelace}
\fi

% ==== local color definitions
\definecolor{CUHKorange}{RGB}{244,106,18} %F47012
\definecolor{CUHKblue}{RGB}{0,111,190}    %006FBE
\definecolor{CUHKgreen}{RGB}{0,127,128}   %007F80
\definecolor{CUHKred}{RGB}{228,46,36}     %E42E24
\definecolor{CUHKyellow}{RGB}{198,148,34} %C69422
\definecolor{CUHKdark}{RGB}{114,44,114}   %722C72
\definecolor{CUHKmiddle}{RGB}{144,44,144} %902C90
\definecolor{CUHKlight}{RGB}{167,44,167} 
\definecolor{CUHKpurple}{RGB}{117,15,109}
\definecolor{CUHKgold}{RGB}{221,163,0}
\definecolor{CUHKribbon}{RGB}{244,223,176}
\definecolor{CUHKblack}{RGB}{34,24,21}

% ==== Local new commands
\newcommand{\etal}{\textit{et al.}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calKL}{\mathcal{KL}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\tool}[1]{$\mathsf{#1}$}
\renewcommand{\bf}[1]{\textbf{#1}}
\renewcommand{\tt}[1]{\texttt{#1}}
\newcommand{\tensor}[1]{\mathcal{#1}}      % define tensor command
\renewcommand{\vec}[1]{\boldsymbol{#1}}    % re-define vec command
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1\right\rvert}}
\newcommand{\mathbbm}[1]{\text{\usefont{U}{bbm}{m}{n}#1}}
\newcommand{\minisection}[1]{\vspace{.06in}\noindent{\textbf{#1}}.}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand\blfootnote[1]{                 % footnote w/o. label
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
\newcommand*\bcircled[1]{                  % black circled
    \tikz[baseline=(char.base)]{
        \node[shape=circle,fill,inner sep=1pt] (char) {\textcolor{white}{#1}};
    }
}
\newcommand*\wcircled[1]{                  % white circled
    \Large{\textcircled{\scriptsize{\textbf{#1}}}}
}


% === beamer style block
\usepackage{tcolorbox}
\tcbuselibrary{skins,breakable}
\newenvironment{myblock}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=white,colframe=CUHKmiddle,%
    colbacklower=white,%
    title=#1]}%
    {\endtcolorbox}
%learn from ChatGPT, automatic add Comment.
\newenvironment{commentblock}[1]{%
    \tcolorbox[beamer,%
    noparskip,breakable,
    colback=white,colframe=CUHKmiddle,%
    colbacklower=white,%
    title=Comment #1]}%
    {\endtcolorbox}


% =============================================================
%              page size setting 
% =============================================================
\iffalse
\paperwidth   = 8.5in                                      % US Letter
\paperheight  = 11.0in
%\paperwidth  = 8.26in                                     % A4
%\paperheight = 11.69in
\usepackage[top=0.78in,bottom=0.86in,left=0.62in,right=0.62in]{geometry}
\setlength{\columnsep}{20pt}                               % set space between columns
\fi
\setlength{\textfloatsep}{10pt plus 1pt minus 1pt}         % set space between float and text
\setlength{\floatsep}{10pt plus 1pt minus 1pt}             % set space between two floats
\setlength{\intextsep}{4pt plus 1pt minus 1pt}             % set space between text and float
\iffalse
\setlength{\abovecaptionskip}{2pt}                         % set space between figure and caption
\setlength{\belowcaptionskip}{2pt}                         % set space between figure and caption
% ==== reduce space around equations
\setlength{\belowdisplayskip}{4pt} \setlength{\belowdisplayshortskip}{4pt}
\setlength{\abovedisplayskip}{4pt} \setlength{\abovedisplayshortskip}{4pt}
% ==== reduce section and subsection title spacing
\newcommand{\subparagraph}{}
\usepackage{titlesec}
\titlespacing*{\section}{0pt}{1.8ex plus .2ex minus .2ex}{0.4ex plus .2ex}
\titlespacing*{\subsection}{0pt}{1.0ex plus .2ex minus .2ex}{0.2ex plus .2ex}
\fi


% =============================================================
%                   Theorem Definitions
% =============================================================
\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mycorollary}{\textbf{Corollary}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myexample}{\textbf{Example}}
\newtheorem{myconjecture}{\textbf{Conjecture}}
\newtheorem{myassumption}{Assumption}
\newtheorem{myprop}{Property}

\crefname{mytheorem}{Theorem}{Theorems}
\crefname{mylemma}{Lemma}{Lemmas}
\crefname{myclaim}{Claim}{Claims}
\crefname{myproperty}{Property}{Properties}
\crefname{mycorollary}{Corollary}{Corollaries}

\algrenewcommand\textproc{\texttt}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% =============================================================
%          Definitions to support latexdiff
% =============================================================
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}{#1}}}                           %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                       %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{}                                                   %DIF PREAMBLE
\providecommand{\DIFaddend}{}                                                     %DIF PREAMBLE
\providecommand{\DIFdelbegin}{}                                                   %DIF PREAMBLE
\providecommand{\DIFdelend}{}                                                     %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                                        %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                                        %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{}                                                 %DIF PREAMBLE
\providecommand{\DIFaddendFL}{}                                                   %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{}                                                 %DIF PREAMBLE
\providecommand{\DIFdelendFL}{}                                                   %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


% =============================================================
%          Local revision functions 
% =============================================================
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}
\newcommand{\revise}[1]{\DIFadd{#1}}

% ==== Logs:
%
%  11/2022: unified setting-ieee
%  05/2021: beamer style block
%  01/2020: todo & revise functions
%  02/2019: vec commend
%  10/2018: captionsetup: remove ":" in caption; eucal package
%  12/2016: titlespacing
%  09/2016: captionsetup
%  07/2016: support to pgfplots
%  07/2016: threeparttable
%  05/2016: setlength intextsep & columnsep
%  04/2016: definitions supporting latexdiff
%  04/2016: remove bookmarks in hyperref
%  02/2016: tabincell
%  02/2016: hyperref
%  12/2015: copy from "ieee_conference"
%


